Fast and Robust Distributed Subgraph Enumeration

We study the classic subgraph enumeration problem under distributed settings. Existing solutions either suffer from severe memory crisis or rely on large indexes, which makes them impractical for very large graphs. Most of them follow a synchronous model where the performance is often bottlenecked by the machine with the worst performance. Motivated by this, in this paper, we propose RADS, a Robust Asynchronous Distributed Subgraph enumeration system. RADS first identifies results that can be found using single-machine algorithms. This strategy not only improves the overall performance but also reduces network communication and memory cost. Moreover, RADS employs a novel region-grouped multi-round expand verify & filter framework which does not need to shuffle and exchange the intermediate results, nor does it need to replicate a large part of the data graph in each machine. This feature not only reduces network communication cost and memory usage, but also allows us to adopt simple strategies for memory control and load balancing, making it more robust. Several heuristics are also used in RADS to further improve the performance. Our experiments verified the superiority of RADS to state-of-the-art subgraph enumeration approaches.

==> Embeddingtrie/embeddingTrie_new_cyctrie.tex <==
\section{Embedding Trie}
\label{sec:embeddingTrie}

\ifpdf
    \graphicspath{{Chapter4/}}
\else
    \graphicspath{{Chapter4/}}
\fi
Recall that in the Algorithm~\ref{algorithm:disSubEnum} of our SubEnum framework, the data structures of cyclic embedding trie $\cycTrie$ and hyper embedding trie $\hypTrie$ plays a significant role in caching the intermediate results ($i.e.$ embedding candidates, assembled embedding IDs). Based on Algorithm~\ref{algorithm:disSubEnum}, it requires that the following requirements should be met: 
\begin{enumerate}[leftmargin=*]
\item[(1)] First and foremost, the data structures should compress those intermediate results to save memory as much as possible. 
\item[(2)] Each item in both $\cycTrie$ and $\hypTrie$ requires a unique ID, by using which we should be able to get and delete the compressed item (We use \textit{item} to refer the compressed embedding or assembled embedding ID). The $\evi$ uses the IDs as keys. Assembled $\hypTrie$ also refers the IDs of items of $\cycTrie$. 


\item[(3)] Given a particular data vertex $v$, $\cycTrie$ requires that we can get a subset of its items where $v$ is mapped to the pivot vertex of the corresponding decomposition unit.

\end{enumerate}
 
With the above requirements in mind, we present details for the $\cycTrie$ and $\hypTrie$ in this section.
 
\subsection{Cyclic Embedding Trie}

 Let us first look at the $\cycTrie$ while before that we need to define a matching order for the query vertices within a decomposition unit $dp_i$, which will be the order of the organized nodes in the $\cycTrie$.

\begin{defn}
  Given a decomposition unit $dp_i$, the matching order $\matchO$ is a relation $\mapsfrom$ between the vertices in $dp_i$ such that
   \begin{enumerate}
   \item $dp_i.u_{pivot} \mapsfrom u$ for all $u\in dp_i.V_{leaf}$.
   \item for any two vertices $u_i, u_j \in dp_i.V_{leaf}$, $u_i\mapsfrom u_j$ if $deg(u_i)$ $>$ $deg(u_j)$, or $deg(u_i) = deg(u_j)$ and the vertex ID of $u_i$ is less than that of $u_j$.
   \end{enumerate}
\label{matchorder}
\end{defn}
The reason that vertices with larger degrees are matched first is that such vertices tend to have fewer candidates in the data graph which may decrease the overall size of $\cycTrie$. $\matchO$($u$) is the order index of query vertex $u$.

Consider the execution plan in Example~\ref{exmp:minimumRounds}, the matching order is $u_0$ $\mapsfrom$ $u_1$ $\mapsfrom$ $u_2$ $\mapsfrom$ $u_9$ $\mapsfrom$ $u_7$ $\mapsfrom$ $u_8$. We have $\matchO$($u_0$)=0 and $\matchO$($u_8$)=5.

With the matching order fixed, we can represent each embedding candidate $\{(u_0, v_0), \ldots, (u_s,v_s)\}$ of $dp_i$ as a list of data vertices $(v_0, \ldots, v_s)$.

Now we are ready to present the definition of the $\cycTrie$.

\ignore{
Given a set of embedding candidates of $dp_i$, suppose the sublist of query vertices is $(u_1, \ldots, u_s)$, we build an inverted trie as follows:
\begin{enumerate}
\item The root of the trie is an empty node, which is at level 0.
\item Each other node  $\trienode$ contains a data vertex $v$ and a pointer that points to the parent of $\trienode$, as well as an integer \textbf{childCount} which represents the number of children of $\trienode$ in the trie.
\item  For $i=1, \ldots, s$, each node in level $i$ corresponds to the query vertex $u_i$, and they are the children of nodes at level $i-1$.

\item The \textbf{childCount} of nodes at level $s$ is 0.
\item The sequence of vertices in the nodes of any root-to-leaf path is an embedding candidate of $P_i$.
\end{enumerate}
}

\begin{defn}
Given a decomposition unit $dp_i$ with its matching order $\matchO$, $\mathcal{R}$ is a set of embeddings or embedding candidates of $dp_i$ in $G_t$, a cyclic embedding trie, denoted as $\cycTrie$, is a multi-level data structure to compress $\mathcal{R}$. And,

\begin{enumerate}
\item[(1)] the depth of $\cycTrie$ is $|\matchO|$.
\item[(2)] $\cycTrie$ contains a list of trie nodes in each level, where each trie node $\trienode$ has 
\begin{itemize}
\item \textbf{id}: a data vertex ID.
\item \textbf{parentN}: a pointer pointing to another trie node.
\item \textbf{childNodeNo}: the total number of trie nodes pointing to $\trienode$.
\end{itemize}
We call the trie nodes in level-0 as headNodes and the ones in level of $(|\matchO|-1)$ as trailNodes.
Only each headNode has an extra field:
\begin{itemize}
\item \textbf{tailNs}: a list of pointers pointing to some tailNodes.
\end{itemize}

\item[(3)] for any query vertex $u$ and any $f\in \mathcal{R}$, there exists a trie node $\trienode$ in the level of $\matchO(u)-1$ such that $\trienode.v$ $=$ $f(u)$.
\item[(4)] for any two query vertices $u$ $\mapsfrom$ $u'$ and any $f\in \mathcal{R}$, there exists one trie node $\trienode$ in the level of $\matchO(u)$ and one trie node $\trienode'$ in the level of $\matchO(u')$ such that: $\trienode'.parentN$ $=$ $\trienode$.
\item[(5)] for any $f\in \mathcal{R}$ and its corresponding headNode $\trienode$ and tailNode $\trienode'$, we have: $\trienode'$ $\in$ $\trienode.tailNs$.

\end{enumerate}
\end{defn}


We set the $childN$ as null for the headNodes.

Given a node $\trienode$ points to $\trienode'$,  $\trienode'$ is called the a $childnode$ of $\trienode$ and $\trienode$ is called as a $parentnode$ of $\trienode'$.   Within the inverted trie, we call the trie nodes without any parentnodes as $tailNodes$.


Intuitively, the $\cycTrie$ applies a hierarchical strategy to group the intermediate results. Given a set of embeddings of query pattern $dp_i$, in the first level, it groups the embeddings by the data vertices mapped to the first query vertex ($i.e.$ pivot) in the matching order. Then for the embeddings falling in the same group of the first level, it groups them by the data vertices mapped to the second query vertex in the matching order. After that the hierarchy goes on until the last query vertex. 

\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.45\textwidth]{pictures/cycTrie}
\caption{Example of Cyclic Embedding Trie}
\label{fig:expandCETrie}
\end{figure}
To easily understand it, see the following example:

\begin{exmp}
Consider a unit $dp_i$ with $V_{dp_i}=\{u_0,$ $u_1,$ $u_2 \}$ and assume we have a matching order $u_0 \mapsfrom u_1 \mapsfrom u_2$, we have an $\cycTrie$ as shown in Figure~\ref{fig:expandCETrie}. The $\cycTrie$ contains 4 items: $\{(v_0, v_2,v_3)$, $(v_0, v_3, v_4)$, $(v_0, v_3,v_5)$, and $(v_1, v_4, v_5)$. The red dotted lines indicate cyclic pointers. 
\end{exmp}


Although the structure of $\cycTrie$ is simple, it elegantly meet the requirements aforementioned.

\ignore{
\begin{algorithm}
\DontPrintSemicolon
\small
\SetAlgoLined
\KwIn{A failed trie node $\trienode$}
$\trienode' \gets \trienode.childN$ \\
\While{$\trienode$ is not Null }
{
		$\trienode'.parentNodeNo--$ \\
		\If{$\trienode'.parentNodeNo$ $= 0$}
		{
			$\trienode'' \gets  \trienode'$
			$\trienode'  \gets \trienode'.childN$       \\
			remove $\trienode''$ from $\invTrie$ \\ 					
		}
}
remove $\trienode$ from $\invTrie$ \\
\caption{\sc removeTrieNode}
\label{algorithm:removeTrieNode}
\end{algorithm}
}

\begin{itemize}[leftmargin=*]
\item \underline{\textit{Compression}} The compression of inverted trie is inherited from the widely known trie structure. Each of our intermediate results accounts for a combination of data vertices. We group the intermediate by the common data vertices in each level so as to reduce the size of intermediate results.

\item \underline{\textit{Unique ID}} For each intermediate result in inverted trie, the location address of its tail node in memory can be used as the unique ID. 

\item \underline{\textit{Get}} Given a particular ID represented by a \emph{tailnode}, we can easily track down its pointer $parentN$ step-by-step to retrieve the corresponding item. Given a data vertex $v$ which is mapped to the $dp_i.u_{pivot}$, first we can track from headNode to its tailNodes according to its cyclic pointers. And then following the pointers of tailNodes, we may get all the corresponding items.

\item \underline{\textit{Delete}}
To remove an item with a particular ID, we can remove its corresponding tailNode and decrease the $childNodeNo$ of its parentNode by 1. If $childNodeNo$ of this parentNode reaches 0, we remove this parentNode. And this process recursively affects its ancestors of the tailNode. 

\ignore{The detailed algorithm is as shown in Algorithm~\ref{algorithm:removeTrieNode}.}

\end{itemize}

Recall Algorithm~\ref{algorithm:disSubEnum} of the SubEnum framework, where a sub-function $expandCETrie()$ is used to construct the $\cycTrie$ of a unit $dp_i$ and its corresponding $\evi$, given a set of candidate vertices of $dp_i.u_{pivot}$. With the definition of $\cycTrie$ ready, now we are ready to present details of this function, as shown in Algorithm~\ref{algorithm:expandCETrie}.

\begin{algorithm}
\DontPrintSemicolon
\small
\LinesNumberedHidden
\SetKwFunction{proc}{proc}
\KwIn{a set of candidate vertices $C_{G_t}(dp_i.u_{pivot})$, unit $dp_i$, local machine $M_t$}
\KwOut{a $\cycTrie$ and $\evi$}

\ShowLn $\matchO$ $\gets$ the matching order of $dp_i$ \\
\ShowLn \For {\textbf{each} $v_{pivot}$ $\in$ $C_{G_t}(dp_i.u_{pivot})$}
	{
\ShowLn init $\cycTrie \gets \emptyset$,  $\evi$ $\gets$ $\emptyset$ \\
\ShowLn create embedding $f \gets \{ (dp_i.u_{pivot}, v_{pivot}) \}$ \\
\ShowLn create an embedding trie node $\trienode$, $\trienode.id \gets $ $v_{pivot}$  \\
\ShowLn	\If{adjEnum($\trienode, u$) returns true}
		{
			push $\trienode$ to $\cycTrie$ \\
		}
	}
%
\setcounter{AlgoLine}{-1}
\SetKwProg{myproc}{Subroutine}{}{}
%
\myproc{adjEnum($\trienode, u$)}
{
\ShowLn $C_{r}(u) \gets Adj(f(dp_i.u_{pivot}))$ \\
\ShowLn \For{each $u'$ mapped in $f$ and $(u, u') \in E_{dp_i}^{sib}$}
		{
\ShowLn		\If{$f(u')$ resides in $M_t$}
			{
\ShowLn			$C_{r}(u) \gets  Adj(f(u')) \cap C_{r}(u)$	\\
			}
		}
			
\ShowLn	\For{\textit{each} $v \in C_{r}(u)$}
		{
\ShowLn		\If{$v$ not mapped in $f$}
			{
\ShowLn			$flag \gets false$ \\
\ShowLn 			create a trie node $\trienode'$ \\
\ShowLn			$\trienode'.id \gets v'$ \\
\ShowLn			$\trienode'.parentN \gets \trienode$ \\
		
\ShowLn			add $(u, v)$ to $f$ \\
\ShowLn			\If{$|f| = |V_{dp_i}|$}
				{
\ShowLn				\For{each undetermined $(v, v')$ of $f$}
					{
\ShowLn					add $\trienode'$ to $\evi[(v, v')]$ \\
					}
\ShowLn				flag $\gets$ true \\
				}
				\Else
				{
\ShowLn				set $u'$ when $\matchO(u') = |f|$  \\
\ShowLn				$flag \gets$ \textit{adjEnum}($\trienode'$, $u'$) \\							
				}
\ShowLn			\If{flag is true}
				{
\ShowLn				$\trienode.childNodeNo++$ \\
\ShowLn				push $\trienode'$ to $\cycTrie$ \\					
				}
\ShowLn		remove $(u, v)$ from $f$ \\	
			}
		}
			
}
\caption{\sc expandCETrie}

\label{algorithm:expandCETrie}
\end{algorithm}

Algorithm~\ref{algorithm:expandCETrie} first compute get matching order of $dp_i$ (Line 1). Then
for each candidate vertex $v$, Algorithm~\ref{algorithm:expandCETrie} initializes a $\cycTrie$ and a $\evi$ as empty (Line 3).  It then creates an embedding $f$ with $v$ being mapped to $dp_i.u_{pivot}$ (Line 4) and creates an embedding trie node $\trienode$ with $v_{pivot}$ as its id (Line 5). After that it calls a subroutine $adjEnum$ to recursively find all the embeddings with $dp_i.u_{pivot}$ being fixed to $v$. If  $adjEnum$ returns true, which means it successfully find some embeddings, we push $\trienode$ to the level-0 of $\cycTrie$.

The \textbf{Subroutine} $adjEnum$ takes a parentNode $\trienode$ and a leaf-vertex $u$ as input. In Line 2 to 4, it refines the candidates for $u$ by considering the recently mapped leaf-vertices of $dp_i$ in $f$ where those leaf-vertices has an edge with $u'$. If the data vertices mapped to those leaf-vertices resides in $M_t$, we shrink the candidates of $u$ by joining it with $Adj(u')$. 
%
Then for each vertex $v$ within refined candidate $C_{r}(u)$, if $v$ has not been used in $f$, we set the flag as false. We then create a new trie node $\trienode'$ with $v$ as its $id$ and point its $parentN$ to $\trienode$ (Line 9, 10). We update $f$ by adding $(u, v)$ to it. And if $u$ is the last leaf of $dp_i$ according to $\matchO$,  we update the $\evi$ by adding the undetermined edges of $f$ to $\evi$ (Line 13, 14) and set a flag to true to indicate we find a embedding candidate in this recursive (Line 15). If $u$ is not the last leaf, we further call the recursive function $adjEnum$ to map the next leaf-vertex according to $\matchO$ (Line 17, 18) and set the flag to true if any partial embedding can be found in deeper recursive.  If there is partial embedding found extending $f$, we increase $childNodeNo$ of $\trienode$ and put the newly created trie node  to $\cycTrie$ (Line 19 to 22). We remove $(u, v)$ from $f$ after trying to map $v$ to $u$ (Line 23).

\subsection{Hyper Embedding Trie}

Now we are ready to study the hyper embedding trie  $\hypTrie$ whose definition is very similar to $\cycTrie$ except for the following two different points:
\begin{enumerate}
\item[(1)] The \textbf{id} field of each trie node in $\hypTrie$ is an ID of an item in $\cycTrie$, which is the location address of a corresponding tailNode.
\item[(2)] $\hypTrie$ does not have the cyclic pointers from headNodes to tailNodes.
\end{enumerate}



Recall Algorithm~\ref{algorithm:disSubEnum}, in the $i^{th}(i>1)$ round, we have the embeddings of $P_{i-1}$ compressed in $\hypTrie$. By assembling with the $\cycTrie$ of unit $dp_i$, we will have the embedding candidates of $P_i$ in the updated $\hypTrie$.
Here we present the details of the assembling function $assembleHETrie$ in Algorithm~\ref{algorithm:assembleHETrie}.

\begin{algorithm}
\DontPrintSemicolon
\small
\SetAlgoLined
\KwIn{embedding $f$, a $\cycTrie$ of unit $dp_i$, a $\hypTrie$, local machine $M_t$}
\KwOut{$\evi$, updated $\hypTrie$}

$v$ $\gets$ $f(dp_i.u_{pivot})$ \\



\For{\textbf{each} machine $M_t$($1\leq t \leq m$) \textbf{simultaneously}}
{
	$\joinplan$ $\gets$ $executionPlan(P)$ \\
	
	$\regiongroup$=$\{rg_0 \dots rg_k\}$ $\gets$ $regionGroups\big(C(dp_0.u_{pivot}, M_t)\big)$ \\
		
	init a list of cyclic embedding tries $\cycTrie$s with size $|\regiongroup|$ \\
	
		
}

\caption{\sc assembleHETrie}
\label{algorithm:assembleHETrie}
\end{algorithm}





==> ExecutionPlan/executionPlan_1.tex <==



\subsection{Computing Execution Plan}
\label{sec:executionPlan}

It is obvious that we may have multiple valid execution plans for a query pattern and different execution plans may have different performance, therefore we want to find the most efficient one among them. In this section, we present some heuristics to find a good execution plan. 

\subsubsection{Minimizing the Number of Rounds}
Given the stripped pattern $\spa$ of query pattern $P$ and an execution plan $\joinplan$, we have { $|\joinplan|+1$} rounds for each region group, and once all the rounds are processed we will get  the set of final embeddings of $\spa$. Also, within each round, the workload can be shared. To be specific, a single undetermined edge $e$ may be shared by multiple {\ec}s.
%For example, consider the subpattern $dp_0$ in Example~\ref{exmp:executionPlan} and the data graph in Figure~\ref{fig:runningExample1}. Suppose $v_{10}$ is on the same machine as $v_0$.
If these embedding candidates are generated in the same round, the verification of $e$ can be shared by all of them. The same applies to the foreign vertices where the cost of fetching and memory space can be shared among multiple embedding candidates if they happen in the same round. Therefore, in order to optimize the performance, our first heuristic is to minimize the number of rounds (namely, the number of decomposition units). Here we present a technique to compute a query execution plan, which guarantees a minimum number of rounds. Our technique is based on the concept of {\em maximum leaf spanning tree} \cite{fernau2011exact}.

\begin{defn}
Given a stripped pattern $\sPattern$, a {\em maximum leaf spanning tree (\mlst)} of $\sPattern$ is a spanning tree of $\sPattern$ with the maximum number of leafs (a leaf is a vertex with degree 1).
The number of leafs in a \mlst of $\sPattern$ is called the {\em maximum leaf number} of $\sPattern$, denoted $l_{\sPattern}$.
\end{defn}

A closely related concept is {\em minimum connected dominating set}.

\begin{defn}
Given a stripped pattern $\sPattern$, a {\em connected dominating set (\cds)}  is a subset $D$ of $V_{\sPattern}$  such that (1) $D$ is a dominating set of $\sPattern$, that is,
any vertex of $\sPattern$ is either in $D$ or adjacent to a vertex in $D$, and (2) the subgraph of $\sPattern$ induced by $D$ is connected.

A {\em minimum connected dominating set (\mcds)} is  a \cds with the smallest cardinality among all \cds{s}.  The number of vertices in a  \mcds is called the {\em connected domination number}, denoted $c_{\sPattern}$.
\end{defn}

It is shown in \cite{MLST92} that \ignore{the set of non-leaf vertices of a \mlst of query $P_{\sPattern}$ is a \mcds  of $P$, therefore} $|V_{\sPattern}|=c_{\sPattern}+l_{\sPattern}$.

\begin{theorem}                                                                                                                                                                                                                         Given a stripped  pattern $\sPattern$, any execution plan of $\sPattern$ has at least $c_{\sPattern}$ decomposition units, and there exists an execution plan with exactly $c_{\sPattern}$ decomposition units.
\label{th1}
\end{theorem}

\begin{proof}
Suppose $\{dp_0, \ldots, dp_k\}$ is an execution plan. The plan has $k+1$ decomposition units. \ignore{According to Definition~\ref{defn:executionPlan},} Clearly the pivot vertices of the decomposition units form a connected dominating set of $\sPattern$. Therefore, $k+1 \geq c_{\sPattern}$. This proves any execution plan has at least $c_{\sPattern}$ decomposition units.

Now suppose $T$ is a \mlst  of $\sPattern$. From $|V_{\sPattern}|=c_{\sPattern}+l_{\sPattern}$ we know the number of non-leaf vertices in $T$ is $c_{\sPattern}$. We can construct an execution plan by choosing one of the non-leaf vertices $v_0$ as $dp_0.\piv$,
and all neighbors of $v_0$ in $T$ as the vertices in $dp_0.\lf$. Regarding $v_0$ as the root of the spanning tree $T$, we then choose each of the non-leaf children $v_i$ of $v_0$ in $T$ as the pivot vertex of the next decomposition unit $dp_i.\piv$,
and all children of $v_i$ as the vertices in $dp_i.\lf$. Repeat this process until every non-leaf vertex of $T$ becomes the pivot vertex of a decomposition unit. This decomposition has exactly $c_P$ units, and it forms an execution plan. This shows that there exists an execution plan with $c_{\sPattern}$ decomposition units.
%
%\ignore{By definition, the expansion edges of $dp_0, \ldots, dp_k$ form a spanning tree $T$ of $P$. Obviously each of the pivot vertices, except $dp_0_piv$,
%must be a non-leaf vertex of $T$, but no others. Thus the number of leaf vertices in $T$, denoted it by $l_T$, is at least $|V_P|-k$. That is, $l_T\geq |V_P|-k$.
%Therefore we have  $l_P\geq |V_P|-k$, which implies $k\geq |V_P|-l_P$, that is $k\geq d_p$.}
\end{proof}

Theorem~\ref{th1} indicates that $c_{\sPattern}$ is the minimum number of rounds of any execution plan. {The above proof  provides a method to construct an execution plan with $c_{\sPattern}$ rounds from a \mlst.} It is worth noting that the decomposition units in the query plan constructed as in the proof have distinct pivot vertices.

\begin{exmp}
Consider the striped pattern $\sPattern$ obtained from the graph $P$ in Figure~\ref{fig:runningExample1}~(a) by eliminating the endvertices $u_7$ and $u_{10}$.
%
It can be easily verified that the tree obtained by erasing the edges $(u_1,u_2)$,  $(u_3, u_4)$, $(u_4,u_5)$, $(u_5,u_6)$ and $(u_8, u_9)$ is a \mlst of $\sPattern$. Choosing $u_0$ as the root, we will get a minimum round execution plan $\joinplan_1$=$\{dp_0$, $dp_1$, $dp_2\}$ where $dp_0.\piv$ $=$ $u_0$, $dp_0.\lf$ $=$ $\{u_1$, $u_2$, $u_8$, $u_9\}$, $dp_1.\piv$ $=$ $u_1$, $dp_1.\lf$ $=$ $\{u_3, u_4\}$ and $dp_2.\piv$ $=$ $u_2$, $dp_2.\lf$ $=$ $\{u_5, u_6\}$.

If we choose $u_1$ as the root, we will get a different minimum-round execution plan $\joinplan_2$=$\{dp_0, dp_1, dp_2 \}$, where
$dp_0.\piv=u_1$, $dp_0.\lf=\{u_0,u_3, u_4\}$,
$dp_1.\piv=u_0$, $dp_1.\lf=\{u_2, u_8,u_9\}$,
$dp_2.\piv = u_2$, $dp_2.\lf=\{u_5, u_6\}$

\label{example4}
\end{exmp}


%\begin{exmp}
%Consider the query pattern $P$ in Figure~\ref{fig:runningExample1}~(a). It can be easily verified that the tree obtained by erasing the edges $(u_1,u_2)$, $(u_8, u_9)$, $(u_3, u_4)$, $(u_4,u_5)$ and $(u_5,u_6)$ is a \mlst of $P$. Choosing $u_0$ as the root, we will get a minimum round execution plan
%$\joinplan_1$=$\{dp_0$, $dp_1$, $dp_2\}$ where $dp_0.\piv$ $=$ $u_0$, $dp_0.\lf$ $=$ $\{u_1$, $u_2$, $u_7$, $u_8$, $u_9\}$, $dp_1.\piv$ $=$ $u_1$, $dp_1.\lf$ $=$ $\{u_3, u_4\}$ and $dp_2.\piv$ $=$ $u_2$, $dp_2.\lf$ $=$ $\{u_5, u_6\}$.
%
%If we choose $u_1$ as the root, we will get a different minimum-round execution plan $\joinplan_2$=$\{dp_0, dp_1, dp_2 \}$, where
%$dp_0.\piv=u_1$, $dp_0.\lf=\{u_0,u_3, u_4\}$,
%$dp_1.\piv=u_0$, $dp_1.\lf=\{u_7,u_2, u_8,u_9\}$,
%$dp_2.\piv = u_2$, $dp_2.\lf=\{u_5, u_6\}$
%
%\label{example4}
%\end{exmp}


\subsection{Moving Forward Verification Edges}
\label{subsec:movingFV}

Given a stripped  pattern $\sPattern$, we may have multiple execution plans with the minimum number of rounds. For example, we can produce different execution plans from the same MLST by choosing different non-leaf vertices as $dp_0.\piv$, and we may also have different MLSTs.  In order to further optimize the performance, we need to find the best plan.
Then the question is: given two execution plans with the same number of rounds, how can we determine one is better than the other?
Here we use a simple heuristic which is to choose plans with more verification edges in the earlier rounds. The intuition is to utilize the filtering power of the verification edges early.
%
To this end, we propose the following score function $\mathcal{SC}(\joinplan)$ for an execution plan $\joinplan=\{dp_0$,  $\dots$,  $dp_{l}\}$:

\begin{equation}
\label{equ:scorePlan}
\mathcal{SC}(\joinplan) = \sum_{dp_i \in \joinplan} \frac{1}{(i + 1)^\rho} \times (|E_{dp_i}^{sib}| + |E_{dp_i}^{cro}|)
\end{equation}
%
Here $|E_{dp_i}^{sib}| + |E_{dp_i}^{cro}|$ is the number of verification edges in round $i$, and $\rho$ is a positive parameter used to tune the score function. In our experiments we use $\rho =1$. The function $\mathcal{SC}(\joinplan)$ calculates a score by assigning larger weights to the verification edges in earlier rounds (since  $\frac{1}{(i + 1)^\rho} > \frac{1}{(j + 1)^\rho}$ if $i<j$).

\begin{exmp}
Consider the query plans $\joinplan_1$ and $\joinplan_2$ in Example~\ref{example4}. The total number of verification edges in these plans are the same. In $\joinplan_1$, the number of verifications edges for the first, second and third round is 2, 1, 2 respectively.  In $\joinplan_2$, the number of verification edges for the three rounds is 1, 2, and 2 respectively. Therefore, we prefer $\joinplan_1$. Using $\rho=1$, we can calculate the scores of the two plans as follows:

$\mathcal{SC}(\joinplan_1)=$ $2/1+ 1/2 + 2/3$ $\approx 3.2$

$\mathcal{SC}(\joinplan_2)=$ $1/1+ 2/2 + 2/3$ $\approx 2.7$

\label{example5}
\end{exmp}

\subsection{Moving Forward Units with Larger Degree Pivots}
\label{subsec:movingFD}

When several minimum-round execution plans have the same score,  we use another heuristic rule to choose the best one from them: the larger the degree of the pivot vertex (in the original pattern instead of the striped pattern), the earlier we process the unit. To accommodate this rule, we can modify the score function in (1) by adding another component as follows:
\begin{equation}
\label{equ:scorePlan1}
\mathcal{SC}(\joinplan)=\sum_{dp_i \in \joinplan}[\frac{|E_{dp_i}^{sib}| + |E_{dp_i}^{cro}|}{(i + 1)^\rho} + \frac{deg(dp_i.\piv)}{(i + 1)}]
\end{equation}


\subsection{Minimizing the span of {$dp_0.piv$}}

Given an execution plan $(dp_0, \ldots, dp_l)$, the starting query vertex is always $dp_0.piv$. Based on Proposition~\ref{lem:diaEmbed}, to maximize the number of embeddings that can be found using \sme, we want to choose $dp_0.piv$ such that it has a minimal span.



%\subsection{Separating end vertices}
%An end vertex is a vertex with degree 1.  In Fig.~\ref{fig:runningExample1}~(a), $u_7, u_8$ and $u_9$ are end vertices.
%End vertices in a query graph can usually be mapped to many vertices in the data graph,


\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.2\textwidth]{Pictures/startVertex}
\caption{A Query Pattern}
\label{fig:embTrie}
\end{figure}



%{Consider two plans ${\joinplan}_1$ and ${\joinplan}_2$ of $5$ rounds. The  number of verification edges in ${\joinplan}_1$ is the same as that in ${\joinplan}_2$, which is equal to the number of edges not in the spanning tree. If the verification edges occur earlier in ${\joinplan}_1$ than in ${\joinplan}_2$ (for instance, most verification edges are in $dp_0, dp_1$ for ${\joinplan}_1$, while most verification edges occur in  $ dp_{4}, dp_5$ for ${\joinplan}_2$), then ${\joinplan}_1$  will have a higher score.}


%Given a query pattern $P$, we may have multiple execution plans with the minimum number of rounds. In order to further optimize the performance, we need to find the
%one with the best performance from them.  Then the question will be: given two execution plans with the same number of rounds, how could we determine one is more efficient than another? To answer this question, we propose the following scoring function $\mathcal{S}(\joinplan)$ for a given plan $\joinplan=\{dp_0$,  $\dots$,  $dp_{l}\}$:
%
%\begin{equation}
%\label{equ:scorePlan}
%\mathcal{SC}(\joinplan) = \sum_{dp_i \in \joinplan} \frac{\rho}{(i + 1)} \times (|E_{dp_i}^{sib}| + |E_{dp_i}^{anc}|)
%\end{equation}
%
%The union of $E_{dp_i}^{sib}$ and $E_{pi}^{anc}$ are the query edges that need to be verified in each round. Our heuristic is to move forward those verification edges so that their filtering power could be put into effect early and the failed candidates can be filtered out early. Function $\mathcal{SC}(\joinplan)$ assigns a score to the unit of each round and sums the score together. The early round $dp_i$ is and the more verification $dp_i$ brings, the higher score $i^{th}$ round will get. A larger $i$ leads to a weak contribution from the verification edges of $dp_i$. Since we index the units from 0, thus the dominator is set as $i$+$1$. $\rho$ is a parameter within a range of $(0, 1)$ to slightly tune up the function.




Based on the above heuristics,  we design an algorithm to compute the execution plan of the query pattern $P$.  The algorithm is shown in Algorithm~\ref{algorithm:computeExecutionPlan} in Appendix~\ref{appendix:computeExecutionPlan}.





==> Experiment/experiement_jw.tex <==
\section{Experiment}
\label{sec:experiment}
In this section, we present our experimental results.

{\stitle{Environment}}
We conducted most our experiments in a cluster platform where each machine is equipped with 16 Intel CPUs and 16G memory. The operating system of the cluster is Red Hat Enterprise Linux 6.5.

{\stitle{Algorithms}}
We compared our system with four other state-of-the-art distributed subgraph enumeration approaches:
\begin{itemize}
\item \psgl \cite{DBLP:conf/sigmod/ShaoCCMYX14}, the algorithm using graph exploration originally based on Pregel.
\item \twintwig\cite{DBLP:journals/pvldb/LaiQLC15}, the algorithm using BFS joining approach originally based on MapReduce.
\item \seed\cite{DBLP:journals/pvldb/LaiQLZC16},  the algorithm using BFS joining approach while supporting clique decomposition unit originally based on MapReduce.
\item \qiao\cite{DBLP:journals/pvldb/QiaoZC17}, the algorithm relying on clique-index and compression and originally using Hadoop system.
\end{itemize}


{\color{blue} Since our system requires custom daemon threads which listen to incoming requests, {where the best implementation is using MPI and socket programming,} we implemented our approach in C++ with the help of Mpich2 \cite{mpich2} and Boost library \cite{boostlibrary}. We used Boost.Asio to achieve the asynchronous message listening and passing. We used TurboIso\cite{turboIso} as our \sme processing algorithm.}

The performance of distributed graph algorithms varies a lot depending on different programming languages and different underline distributed engine and file systems \cite{DBLP:journals/pvldb/AmmarO18}. It is not fair enough to simply compare our approach with the Pregel-implemented \psgl or  other Hadoop-based approaches. Therefore to achieve a fair comparison, we implemented \psgl, \twintwig and \seed  using C++ with MPI library. {\color{red} For \qiao, we chose to use the original program provided by its authors mainly because of the complexity of its implementation.} In memory, we loaded the data graph in each node in the format of adjacency-list for \Pads, \psgl and \twintwig. In order to support the clique decomposition unit of \seed, we also loaded the edges in-memory between the neighbours of a vertex along with the adjacency-list of the vertex.

{\stitle{Dataset \& Queries}} We used four real datasets in our experiments: DBLP, RoadNet, LiveJournal and UK2002.  The profiles of these data sets are given in Table~\ref{t:datasets}. The diameter in Table~\ref{t:datasets} is the longest shortest path between any two data vertices. We partitioned each data graph using the multilevel k-way partition algorithm provided by Metis \cite{metis}. DBLP is a relatively small data graph which can be loaded into memory without partitioning, however, we still partition it here. One may argue when the data graph is small, we can use single-machine enumeration algorithms. However, our purpose of using DBLP here is not to test which algorithm is better when the graph can be loaded as a whole, but is to test whether the distributed approaches can fully utilize the memory when there is enough space available.

{\color{blue} RoadNet is a larger but much sparser data graph than the others,  consequently the number of embeddings of each query is smaller. Therefore it can be used to illustrate whether a subgraph enumeration solution has good filtering power to filter out false embeddings early. In contrast, the two denser data graphs, liveJournal and UK2002, are used to test the algorithms' ability to handle denser graphs with huge numbers of embeddings.}

\begin{table}[h]
    \caption{Profiles of datasets}
	\centering
	\label{t:datasets}
 	\begin{tabular}{|c|c|c|c|c|}
    \hline
     \textbf{Dataset($G$)} & $ |V| $ & $ |E| $  & Avg. degree & Diameter \\ \hline \hline
     \textbf{RoadNet}     &  56M    & 717M      & 1.05        & 48K  \\ \hline   	
   	 \textbf{DBLP}        &  0.3M   & 1.0M      & 6.62        & 21   \\ \hline
   	 \textbf{LiveJournal} &  4.8M   & 42.9M     & 18          & 17 \\ \hline
   	 \textbf{UK2002}      &  18.5M  & 298.1M    & 32          & 22 \\ \hline
	\end{tabular}
\end{table}

On disk, our data graphs are stored in plain text format where each line represents an adjacency-list of a vertex. The approach of \qiao relies on the clique-index of the data graph which should be pre-constructed and stored on disk. In Table~\ref{t:qiao_index}, we present the disk space cost of the index files generated by the program of \qiao (M for Mega Bytes, G for Giga Bytes).

\begin{table}[h]
    \caption{Illustration of the Size of Index Files of \qiao}
	\centering
	\small
	\label{t:qiao_index}
 	\begin{tabular}{|c|c|c|c|c|}
    \hline
     \textbf{Dataset($G$)} & Data Graph File Size & Index File Size \\ \hline \hline
   	 \textbf{DBLP}   & 13M   & 210M   \\ \hline
     \textbf{RoadNet} & 2.3G   & 16.9G     \\ \hline
   	 \textbf{LiveJournal}   & 501M   & 6.5G   \\ \hline
   	 \textbf{UK}   & 4.1G   & 60G   \\ \hline
	\end{tabular}
\end{table}


The queries we used are given in Figure~\ref{fig:query1}.

\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.45\textwidth]{Pictures/query1}
\caption{Query Sets}
\label{fig:query1}
\end{figure}



We evaluate the performance, measured by time elapsed and communication cost, of the five approaches in Section~\ref{subsec:performanceCom}. The cluster we used for this experiment consists of 10 nodes. Due to space limit, more experimental results, including execution plan evaluation and scalability test etc., are presented in Appendix~\ref{appendix:moreResults}.


\subsection{Performance Comparison}
\label{subsec:performanceCom}



We compare the performance of five subgraph enumeration approaches by measuring the time elapsed (in seconds) and the volume of exchanged data of processing each query pattern. The results of DBLP, RoadNet, LiveJournal and UK2002 are given in \ref{fig:10_roadnet}, Figure~\ref{fig:10_dblp},  Figure~\ref{fig:10_livejournal} and Figure~\ref{fig:10_uk} , respectively. We mark the result as empty when the test fails due to out-of-memory errors. When any bar reaches the upper bound, it means the corresponding values is beyond the upper bound value shown in the chart.



\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_roadNet}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_roadNet}
         \caption{Communication Cost}
      \end{subfigure}
	\caption{Performance over RoadNet}
	\label{fig:10_roadnet}
\end{figure}


\stitle{Exp-1:RoadNet}
The results over the RoadNet dataset is given in Figure~\ref{fig:10_roadnet}~(a). As can be seen from the figure, \Pads and \psgl are significantly faster than the other three methods (more than 1 order of magnitude). \Pads and \psgl are using graph exploration while the others are using join-based methods. Therefore, both \Pads and \psgl demonstrated efficient filtering power. Since join-based methods need to group the intermediate results based on keys so as to join them together, the performance was significantly dragged down when dealing with sparse graphs compared with \Pads and \psgl.

It is worth noting that \psgl was verified slower than \twintwig and \seed in \cite{DBLP:journals/pvldb/LaiQLC15}\cite{DBLP:journals/pvldb/LaiQLZC16}. This  may be  because the datasets used in \twintwig and \seed are much denser than roadNet, where a huge number of embeddings will be generated. The grouped intermediate results of \twintwig and \seed significantly reduced the cost of network traffic. Another interesting observation is that although \qiao has heavy indexes, its performance is much worse than \psgl and \Pads.
%
{\color{red} The reason is that the number of cliques in RoadNet is relatively small considering the graph size. \ignore{This indicates the performance of \qiao is highly affected by the type of data graphs.} Moreover, there are no crystals {\color{red} (core?)} with more than one vertex  in queries $q_1$, $q_3$, $q_6$, $q_7$ and $q_8$. In such cases,
\ignore{the method of \qiao is similar to the other two join-methods with each decomposition unit being an edge.} the clique indexes cannot help to improve the performance.
%But for $q_6$ $q_7$ and $q_8$ \qiao is still much better than SEED, why?

As shown in Figure~\ref{fig:10_roadnet}(b), the communication cost is not large for all the approaches (less than 5M for most queries). In particular, for  \Pads, the communication cost is almost 0 which is mainly because most data vertices can be processed by \sme, as such no network communication is required. 


\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_dblp}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_dblp}
         \caption{Communication Cost}
      \end{subfigure}

	\caption{Performance over DBLP}
	\label{fig:10_dblp}
\end{figure}

\stitle{Exp-2:DBLP} The result over DBLP is shown in Figure~\ref{fig:10_dblp}.
As aforementioned, DBLP is smaller but much denser than RoadNet. The number of intermediate results generated in DBLP are much larger than that in RoadNet, as implied by the data communication cost shown in Figure~\ref{fig:10_dblp}~(b).
Since \psgl does not consider any compression or grouping over intermediate results, the communication cost of \psgl is much higher than the other approaches (more than 200M for queries after $q_4$).  Consequently, the time delay due to shuffling the intermediate results caused bad performance for \psgl. However, \psgl is still faster than \seed and \twintwig. This may be because the time cost of grouping intermediate results of \twintwig and \seed is heavy as well. It is worth noting that the communication cost of our \Pads is quite small (less than 5M). This is because of the caching strategy of \Pads where most foreign vertices are only fetched once and cached in the local machine. If most vertices are cached, there will be no further communication cost. The time efficiency of \Pads is better than \qiao even for queries $q_2$,$q_4$ and $q_5$ where the triangle crystal can be directly loaded from index without any computation.


\stitle{Exp-3:LiveJournal} As shown in Figure~\ref{fig:10_livejournal}, for LiveJournal, \seed, \twintwig and \psgl start becoming impractical for queries from $q_3$ to $q_8$. It took them more than 10 million seconds in order to process each of those queries. Due to the huge number of intermediate results generated, the communication cost increased significantly as well, especially for \psgl whose communication cost was beyond control when the query vertices reach 6. The method of \qiao achieved a good performance for queries $q_2$, $q_4$ and $q_5$. This is mainly because \qiao simply retrieved the cached embeddings of the triangle to match the vertices $(u_0,u_1,u_2)$ of those 3 queries. However, when dealing with the queries with no good crystals ($q_6$, $q_7$ and $q_8$), our method significantly outperformed \qiao (by almost halving the processing time). One important thing to note is that the other three methods (\seed, \twintwig and \psgl) are sensitive to the end vertices, such as $u_5$ in $q_5$. Both time cost and communication cost increased significantly from $q_4$ to $q_5$. \Pads processes those end vertices last by simply enumerating the combinations without caching any results related to them. The end vertices within \qiao will be bud vertices which only requires simple combinations. As indicated by query $q_5$ where their processing time increased slightly from that of $q_4$, \Pads and \qiao are nicely tuned to handle end vertices.

\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_livejournal}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_livejournal}
         \caption{Communication Cost}
      \end{subfigure}

	\caption{Performance over LiveJournal}
	\label{fig:10_livejournal}
\end{figure}
	
\stitle{Exp-4:UK2002}
As shown in Figure~\ref{fig:10_uk}, \twintwig, \seed and \psgl failed the tests of queries after $q_3$ due to memory failure caused by huge number of intermediate results. The communication cost of all other methods are significantly larger than \Pads (more than 2 orders of magnitude), we omit the chart for communication cost here. Similar to that of LiveJournal, the processing time of \qiao is better than that of \Pads for the queries with cliques. This is because  \qiao directly retrieves the embeddings of the cliques from the index. However, for queries without good crystals, our approach demonstrates better performance. As shown in Table~\ref{t:qiao_index}, the index files of \qiao is more than 10 times larger than the original data graph. Another advantage of \Pads over \qiao is our memory control strategies ensures it is more robust: we tried to set a memory upper bound of 8G and test query $q_6$, \qiao starts crashing due to memory leaks,  while \Pads successfully finished the query for this test.

\begin{figure}[htbp!]		
   \centering
   \includegraphics[width=0.5\textwidth]{Pictures/Experiment/10_time_uk2002}
   \caption{Time cost over UK2002}
   \label{fig:10_uk}
\end{figure}
	
	


==> Experiment/experiment_old.tex <==
\section{Experiment}
\label{sec:experiment}
In this section, we present our experimental results.

{\stitle{Environment}}
We conducted most our experiments in a cluster platform where each machine is equipped with 16 Intel Xeon CPUs and 16G memory. The operating system of the cluster is Red Hat Enterprise Linux 6.5.

{\stitle{Algorithms}}
We compared our system with four other state-of-the-art distributed subgraph enumeration approaches:
\begin{itemize}
\item \psgl \cite{DBLP:conf/sigmod/ShaoCCMYX14}, the algorithm using graph exploration originally based on Pregel.
\item \twintwig\cite{DBLP:journals/pvldb/LaiQLC15}, the algorithm using BFS joining approach originally based on MapReduce.
\item \seed\cite{DBLP:journals/pvldb/LaiQLZC16},  the algorithm using BFS joining approach while supporting clique decomposition unit originally based on MapReduce.
\item Qiao\cite{DBLP:journals/pvldb/QiaoZC17}, the algorithm relying on clique-index and compression and originally using Hadoop system.
\end{itemize}


Since our system \Pads requires custom daemon threads listening out-coming requests whose best implementation solution is using MPI and socket programming. Therefore, we implemented our approach in C++ with the help of Mpich2 \cite{mpich2} and Boost library \cite{boostlibrary}. We used Boost.Asio to achieve the asynchronous message listening and passing. We used TurboIso\cite{turboIso} as our \sme processing algorithm.

The performance of distributed graph algorithm varies a lot considering different programming languages and different underline distributed engine and file systems \cite{DBLP:journals/pvldb/AmmarO18}. It is not fair enough to simply compare our approach with the Pregel-implemented \psgl or  other hadoop based approaches. Therefore to achieve a fair comparison, we implemented \psgl, \twintwig and \seed by using C++ with MPI library. While considering the complexity of Qiao, we finally chose to use the program provided by its original authors. In memory, we loaded the data graph in each node in the format adjacency-list for \Pads, \psgl and \twintwig. In order to support the clique decomposition unit of \seed, we also loaded the edges in-memory between the neighbours of a vertex along with the adjacency-list of the vertex.

{\stitle{Dataset \& Queries}} We used four real datasets in our experiments: DBLP, Roadnet, LiveJournal and UK whose profiles are given in Table~\ref{t:datasets}. The diameter in Table~\ref{t:datasets} is the longest shortest path between any two data vertices. We partitioned each data graph using the multilevel k-way partition algorithm provided by Metis \cite{metis}. The DBLP is a relatively small data graph which can be loaded into the memory without partitioning, however, we still partitioned it here. One may argue when the data graph is small, we can use single-machine enumeration algorithms. However, our purpose of using DBLP here is not to say which algorithm is better when the graph can be loaded as a whole, but is to test whether the distributed approaches can fully utilize the memory when there is enough space available.

RoadNet is a relatively larger while much sparser data graph than the others where consequently the number of embeddings of each query will be smaller. Therefore it can be used to illustrate whether a subgraph enumeration solution has a good filtering technique to filter out false embeddings at early state. In contrast, the two denser data graphs of liveJournal and UK2002 are good indicator of the algorithms' ability of handling larger graphs with huge number of embeddings.

\begin{table}[h]
    \caption{Profiles of datasets}
	\centering
	\label{t:datasets}
 	\begin{tabular}{|c|c|c|c|c|}
    \hline
     \textbf{Dataset($G$)} & $ |V| $ & $ |E| $  & Avg. degree & Diameter \\ \hline \hline
     \textbf{RoadNet}     &  56M    & 717M      & 1.05        & 48K  \\ \hline   	
   	 \textbf{DBLP}        &  0.3M   & 1.0M      & 6.62        & 21   \\ \hline
   	 \textbf{LiveJournal} &  4.8M   & 42.9M     & 18          & 17 \\ \hline
   	 \textbf{UK2002}      &  18.5M  & 298.1M    & 32          & 22 \\ \hline
	\end{tabular}
\end{table}

In the disk, our data graphs are stored in plain text format where each line represents an adjacency-list of a vertex. The approach of Qiao relies on the clique-index of the data graph which should be pre-constructed and stored in disk. In Table~\ref{t:qiao_index}, we present the disk space cost of the index files generated by the program of Qiao (M for Mega Bytes, G for Giga Bytes).

\begin{table}[h]
    \caption{Illustration of the Size of Index Files of Qiao}
	\centering
	\small
	\label{t:qiao_index}
 	\begin{tabular}{|c|c|c|c|c|}
    \hline
     \textbf{Dataset($G$)} & Data Graph File Size & Index File Size \\ \hline \hline
   	 \textbf{DBLP}   & 13M   & 210M   \\ \hline
     \textbf{RoadNet} & 2.3G   & 16.9G     \\ \hline
   	 \textbf{LiveJournal}   & 501M   & 6.5G   \\ \hline
   	 \textbf{UK}   & 4.1G   & 60G   \\ \hline
	\end{tabular}
\end{table}


The queries we used are given in Figure~\ref{fig:query1}.

\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.45\textwidth]{Pictures/query1}
\caption{Query Sets}
\label{fig:query1}
\end{figure}



We evaluate the performance, measured by time elapsed and communication cost, of the five approaches in Section~\ref{subsec:performanceCom}. The cluster of this section consists of 10 nodes. Due to space limit, more experiments results, including execution plan evaluation and scalability test etc., are presented in Appendix~\ref{appendix:moreResults}.


\subsection{Performance Comparisons}
\label{subsec:performanceCom}



We compare the performance of five subgraph enumeration approaches by measuring the time elapsed (in seconds) and the volume of exchanged data of processing each query pattern. The results of DBLP, Roadnet, LiveJournal and UK2002 are given in \ref{fig:10_roadNet}, Figure~\ref{fig:10_dblp},  Figure~\ref{fig:10_livejournal} and Figure~\ref{fig:10_uk} , respectively. We mark the result as empty when any test failed due to out-of-memory errors. When any bar reaches to the upper bound, it means the corresponding values is beyond the upper bound value shown in the chart.



\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_roadNet}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_roadNet}
         \caption{Communication Cost}
      \end{subfigure}

	\caption{Performance over Roadnet}
	\label{fig:10_roadnet}
\end{figure}


\stitle{Exp-1:Roadnet}
Let us first look at the results over Roadnet dataset in Figure~\ref{fig:10_roadnet}(a), where the time efficiency of \Pads and \psgl are significantly faster than the other three methods (more than 1 order of magnitude). \Pads and \psgl are using graph exploration while the others are using join-based methods. Therefore, toth \Pads and \psgl demonstrated efficient filtering power. Since join-based methods need to group the intermediate results based on keys so as to join them together, the performance was significantly dragged down when dealing with sparse graphs compared with \Pads and \psgl.

It is worth noting that \psgl was verified slower than \twintwig and \seed in \cite{DBLP:journals/pvldb/LaiQLC15}\cite{DBLP:journals/pvldb/LaiQLZC16}. This is because the datasets used in \twintwig and \seed are much denser than roadNet, where a huge number of embeddings will be generated. The grouped intermediate results of \twintwig and \seed significantly reduced the time cost of network traffic. Another interesting find is that although Qiao utilized heavy indexes, its performance is much worse than \psgl and \Pads. The reason is obvious, the number of cliques of Roadnet is small which indicates the performance of Qiao is highly affected by the type of data graphs. Moreover, there are no crystals with more than one vertex existing in query $q_1$, $q_3$, $q_6$, $q_7$ and $q_8$. Under such situations, the method of Qiao is similar to the other two join-methods with each decomposition unit being an edge. The clique-indexes cannot help to improve the performance.

Figure~\ref{fig:10_roadnet}(b), the communication cost is not large for all the approaches (less than 5M for most queries). Especially for our \Pads, the communication cost is almost 0 which mainly because most data vertices can be processed by \sme where no communication cost is generated.


\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_dblp}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_dblp}
         \caption{Communication Cost}
      \end{subfigure}

	\caption{Performance over DBLP}
	\label{fig:10_dblp}
\end{figure}

\stitle{Exp-2:DBLP} Next let us look at the results over DBLP.
As aforementioned, DBLP is a small data graph while much denser than Roadnet. The volume of embeddings and intermediate results generated in DBLP are much larger than that in Roadnet, as shown in Figure~\ref{fig:10_dblp}(b). Since \psgl has not considered any compression nor grouping over intermediate results, the communication cost of \psgl is much higher than the other approaches (more than 200M for queries after $q_4$).  Consequently, the time legacy due to shuffling those intermediate results lead a bad performance for \psgl. However, \psgl is still faster than Seed and Twintwig. This may because the time cost of grouping intermediate results of \twintwig and \seed is heavy as well. It is worth noting to note that the communication cost of our \Pads is quite small (less than 5M). This is because of the caching strategy of \Pads where most foreign vertices are only fetched once and cached in the local machine. If most vertices are cached, there will be no further communication cost. The time efficiency of \Pads is better than Qiao even for queries $q_2$,$q_4$ and $q_5$ where the triangle crystal can be directly loaded from index without any computation.


\stitle{Exp-3:LiveJournal}
As for LiveJournal, \seed, \twintwig and \psgl start becoming impractical for queries from $q_3$ to $q_8$. It took them more than 10000 thousands seconds in order to process those queries. Due to a huge number of intermediate results were generated, the communication cost of them increased significantly as well. Especially for \psgl whose communication cost was beyond control when the query vertices reach 6. The method of Qiao achieved a good performance for queries $q_2$, $q_4$ and $q_5$. This is mainly because Qiao simply retrieved the cached embeddings of the triangle to match the vertices $(u_0,u_1,u_2)$ of those 3 queries. However, when dealing with the queries with no good crystals ($q_6$, $q_7$ and $q_8$), our method significantly outperformed Qiao by almost half less of the processing time. One important thing to note is that the other three methods (\seed, \twintwig and \psgl) are sensitive to the end vertices with degree as one, such as $u_5$ in $q_5$. Both time cost and communication cost increased significantly from $q_4$ to $q_5$. \Pads process those end vertices at last by simply enumerating the combinations without caching any results related to them. The end vertices within Qiao will be bud vertice which only requires simple combinations. Just as indicated by query $q_5$ where their processing time increased slightly, those two methods are nicely tuned to handle end vertices.

\begin{figure}[htbp!]		
      \centering
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_time_livejournal}
		\caption{Time cost}
      \end{subfigure} \\%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
      \begin{subfigure}[b]{0.5\textwidth}
    		\includegraphics[width=\textwidth]{Pictures/Experiment/10_commu_livejournal}
         \caption{Communication Cost}
      \end{subfigure}

	\caption{Performance over LiveJournal}
	\label{fig:10_livejournal}
\end{figure}
	
\stitle{Exp-4:UK2002}
As shown in Figure~\ref{fig:10_uk}, \twintwig, \seed and \psgl failed the tests of queries after $q_3$ due to memory failure caused by huge number of intermediate results. The communication cost of all other methods are significantly larger than \Pads (more than 2 orders of magnitude), we omit the chart for communication cost here. Similar to that of LiveJournal, the processing time of Qiao is better than that of \Pads for the queries with cliques. It is admitted that the time saving through directly retrieving the cliques from the pre-index cliques significantly reduce the online query processing time. However, considering the queries without good crystals for Qiao, our approach demonstrates better performance. As shown in Table~\ref{t:qiao_index}, the index files of Qiao is more than 10 times larger than the original data graph. We tried to set an upper bound memory limit as 8G and test query $q_6$, Qiao starts crashing due to memory leaks. While \Pads successfully finished the query under this test.

\begin{figure}[htbp!]		
   \centering
   \includegraphics[width=0.5\textwidth]{Pictures/Experiment/10_time_uk2002}
   \caption{Time cost over UK2002}
   \label{fig:10_uk}
\end{figure}
	
	


==> Optimization/optimization.tex <==
\section{Optimization strategies} 
This section presents our optimization strategies. 

\subsection {Handling end vertices separately}
Since the embeddings of $P$ can be obtained from those of $\sp$ with a simple Cartesian expansion process, in \Mur we choose to process $\spa$ first. That is, on each machine, for the candidate vertices of $dp_0.piv$ that cannot be processed by \sme, we will first process $\spa$, then expand the embeddings of $\spa$ into that of $P$. This will help save memory since we do not need to cache the candidate vertices  of the end vertices. Note that the Cartesian expansion process may need to fetch foreign vertices.



    

==> Outline/embeddingTrie_1.tex <==
\section{Embedding Trie}
\label{sec:embeddingTrie}
%Recall that in Algorithm~\ref{algorithm:disSubEnum} of our framework, the  data structure \embTrie
%plays an important role in caching intermediate results (i.e., embebdings and \ec{s}).
%
%To save memory and facilitate edge verification it should meet the following requirements:
%\begin{enumerate}[leftmargin=*]
%\item[(1)] be able to compress the intermediate results.
%\item[(2)] support easy insertion, removal, and retrieval of intermediate result, and be {\em dynamic}: grow or shrink with the number of intermediate results in it.
%\item[(3)] provide each individual intermediate result with a simple unique ID.
%\end{enumerate}
%
%\noindent With  these requirements in mind, we propose a trie-like data structure named \textit{embedding trie} in this section.

In this section we present the \textit{embedding trie} and its related algorithms. For brevity, we will use {\em result} to refer to an embedding or an embedding candidate.

\subsection{Matching order and merged result lists}

We first define a matching order, which is the order following which the query vertices are matched in \Mur. It is also the order the nodes in the \et are organized.
{
\begin{defn}[Matching Order]
  Given a query execution plan  $\joinplan$ $=$ $\{dp_0$, $\ldots$, $dp_l\}$ of stripped pattern  $\sPattern$, the matching order w. r. t $\joinplan$ is a relation  $\prec$  defined over the vertices of $P$ that satisfies the following conditions:
   \begin{enumerate}
   \item $dp_i.piv \prec$ $dp_j.piv$ if $i<j$;
   \item For any two vertices $u_1\in dp_i.\lf$ and $u_2\in dp_{j}.\lf$, $u_1\prec u_2$ if $i<j$.
   %\item For any two vertices $u_1\in dp_i$ and $u_2\in dp_{j}$, $u_1\prec u_2$ if $i<j$ and $u_2 \notin P_{i}$. %for  %is not the pivot vertex of $dp_j$ which is also in $dp_k.\lf$ where $k<i$.

   \item For  $i\in[0,l]$:
	\begin{enumerate}[label = (\roman*)]
	\item $dp_i.\piv\prec u$ for all $u\in dp_i.\lf$;
	\item for  any vertices $u_1$, $u_2\in dp_i.\lf$ that are not the pivot vertices of other units,  $u_1\prec u_2$ if $deg(u_1)$ > $deg(u_2)$, or $deg(u_1) = deg(u_2)$ and the vertex ID of $u_1$ is less than that of $u_2$;
	\item if $u_1\in dp_i.\lf$ is a pivot vertex of another unit, and $u_2\in dp_i.\lf$ is not a pivot vertex of another unit, then $u_1\prec u_2$.
    \end{enumerate}	
   \end{enumerate}
\label{matchorder}
\end{defn}

Intuitively the above relation orders the vertices of $P$ as follows:
(a) Generally a vertex $u_1$ in $dp_i$ is before a vertex $u_2$ in $dp_j$ if $i<j$, except for the special case where $u_1\in dp_i.\lf$ and $u_2=dp_j.piv$. In this special case, $u_2$ may appear in the leaf of some previous unit $dp_k$ ($k\leq i$), and it may be arranged before $u_1$ according to Condition (2) or Condition (3) (ii).
%
\ignore{$dp_j.\piv$ if $dp_j.\piv$ is a leaf vertex of some $dp_k$ ($k\leq i$), in which case its position has been determined when the leaves of $dp_k$ are arranged.}
(b) Starting from $dp_0$, the vertex $dp_0.\piv$ is arranged before all other vertices. For the leaf vertices of $dp_0$, it arranges those that are pivot vertices of other units before those that are not (Condition (3)(iii)), and for the former, it arranges them according to the ID of the units for which they are the pivot vertex\footnote{Note that no two units share the same pivot vertex.} (Condition (1)); for the latter, it arranges them in descending order of their degree in the original pattern $P$, and if they have the same degree it arranges them in the order of vertex ID (Condition (3) (ii)).
For each subsequent $dp_i$, the pivot vertex must appear in the leaf of some previous unit, hence its position has been fixed; and the leaf vertices of $dp_i$ are arranged in the same way as the leaf vertices of $dp_0$.
}%\color

It is easy to verify $\prec$ is a strict total order over $V_P$. Following the matching order, the vertices of $P$ can be arranged into an ordered list.
Consider the execution plan $\joinplan_1$ in Example~\ref{example4}. The vertices in the query can be arranged as $u_0, u_1,u_2,u_8,u_9,u_3,u_4,u_5,u_6$ according to the matching order.

%For easy presentation, we assume the query vertices have been arranged into the list $u^0, u^1, \ldots, u^n$ , that is, the vertex at position $j$ is $u^j$, and we use $L_P$ to denote the list.

Let $\joinplan=\{dp_0$, $\ldots$, $dp_l\}$ be an execution plan,  $P_i$ be the subgraph of $P$ induced from the vertices in $dp_0\cup \cdots \cup dp_i$ (as defined in Section~\ref{subsec:rmeef}), and $\mathbb{R}$ be a set of {\em results} (can be embeddings or embedding candidates) of $P_i$.  For easy presentation, we assume the vertices in $P_i$ has been arranged into the list $u^0, u^1, \ldots, u^n$ by the matching order, that is, the query vertex at position $j$ is $u^j$. Then each result of $P_i$ can be represented as a list of corresponding data vertices.   These lists can be merged into a collection of trees as follows:

\begin{enumerate}
\item[(1)] Initially, each result $f$ is treated as a tree $T_f$, where the node at level $j$ stores the data vertex $f(u^j)$ for $j\in [0,n]$, and the root is the node at level 0.

\item[(2)] If multiple results map $u^0$ to the same data vertex, merge the root nodes of their trees. This partitions the results in $\mathbb{R}$ into different groups, each group will be stored in a distinct tree.

%\item[(3)] For each tree generated above, if several children of the root store the same data vertex,  merge these children into a single child of the root.

\item[(3)] For each newly merged node $\trienode$, if multiple children of  $\trienode$ correspond to the same vertex, merge these children into a single child of $\trienode$.

\item[(4)] Repeat step (3) untill no nodes can be merged.
\end{enumerate}

The collection of trees obtained above is a compact representation of the results in $\mathbb{R}$. Each leaf node in the tree uniquely identifies a result.
%Obviously storing the results $\mathbb{R}$ using the above trees can save space.

The embedding trie is a collection of similar trees. However, since the purpose of the embedding trie is to save space, we cannot get it by merging the result lists. Instead, we will have to construct it by inserting nodes one by one when results are generated, and removing nodes when results are eliminated. Next we formally define \et  and present the algorithms for the maintenance of the \et.

\subsection{Structure of the Embedding Trie}

\begin{defn}[Embedding Trie]
 Given a set $\mathbb{R}$ of results of $P_{i}$, the {\em embedding trie} of $\mathbb{R}$ is a collection of trees used to store the results in $\mathbb{R}$ such that:
\begin{enumerate}
 \item Each tree represents a set of results that map $u^0$ to the same data vertex.

 \item Each tree node $\trienode$ has
    \begin{itemize}
    \item \textbf{v}:  a data vertex
    \item \textbf{parentN}:   a pointer pointing to its parent node (the pointer of the root node is null).

    \item \textbf{childCount}: the number of child nodes of $\trienode$.
    \end{itemize}

\item If two nodes have the same parent, then they store different data vertices.

\item Every leaf-to-root path represents a result in $\mathbb{R}$, and every result in $\mathbb{R}$ is represented as a unique leaf-to-root path.

\item If we divide the tree nodes into different levels such that the root nodes are at level 0, the children of the root nodes are at level 1 and so on, then the tree nodes at level $j$ ($j\in [0,1]$) store the set of values $\{f(u^j) | f\in$ $\mathbb{R}$ $\}$.
\end{enumerate}

\end{defn}

%Because of condition (4), we can use the corresponding leaf node as the ID of the result.


%For any $u\in V_{P_i}$, we define $\mathbb{R}(u)=\{ f(u) | f\in \mathbb{R} \}$.
%
%(1) starting from $u^0$, for each data vertex $v^0$ in $\mathbb{R}(u^0)$ create a node $\trienode$ such that $\trienode.v = v^0$.
%
%(2) for each data vertex in $\mathbb{R}(u^1)$, create a child node $\trienode'$ of $\trienode$ if and only if there is $f\in \mathbb{R}$ such that $f(u^1)=$
%
%(2) For each node $\trienode$ created above, create a child node $\trienode'$ of For every  $f\in \mathbb{R}$, if $f(u^1)$
%

\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.45\textwidth]{Pictures/embTrie}
\caption{Example of Embedding Trie}
\label{fig:embTrie}
\end{figure}

%To easily understand it, see the following example:

\begin{exmp}
Consider $P_0$ in Example~\ref{exmp:runningExmp}, where the vertices are ordered as $u_0,u_1, u_2$ according to the matching order. There are three \ec{s} of $P_0$: $(v_0,v_1,v_2)$, $(v_0,v_1,v_9)$ and $(v_0,v_9,v_{11})$. These results can be stored in a tree shown in   Figure~\ref{fig:embTrie}(a).
 %
When the second \ec is filtered out, we have $\mathbb{R}_{G_t}(P_{0})$ compressed in a tree as shown in Figure~\ref{fig:embTrie}(b).
The first \ec can be expanded to an \ec of $P_1$ (where the list of vertices of $P_1$ are $u_0, u_1,u_2,u_3,u_4$), which is as shown in Figure~\ref{fig:embTrie}(c).
\end{exmp}



%Although the structure of \embTrie is simple, it elegantly meet the requirements aforementioned.

\ignore{
\begin{algorithm}
\DontPrintSemicolon
\small
\SetAlgoLined
\KwIn{A failed trie node $\trienode$}
$\trienode' \gets \trienode.childN$ \\
\While{$\trienode$ is not Null }
{
		$\trienode'.parentNodeNo--$ \\
		\If{$\trienode'.parentNodeNo$ $= 0$}
		{
			$\trienode'' \gets  \trienode'$
			$\trienode'  \gets \trienode'.childN$       \\
			remove $\trienode''$ from $\invTrie$ \\ 					
		}
}
remove $\trienode$ from $\invTrie$ \\
\caption{\sc removeTrieNode}
\label{algorithm:removeTrieNode}
\end{algorithm}
}

Although the structure of embedding trie is simple,  it has some nice properties:

\begin{itemize}[leftmargin=*]
\item \underline{\textit{compression}} Storing the results in the \et saves space than storing them as a collection of lists.

%The compression of embedding trie is inherited from the widely known trie structure. Each of our intermediate results accounts for a combination of data vertices. We group the intermediate results by the common data vertices in each level so as to reduce the size of intermediate results.

\item \underline{\textit{Unique ID}} For each result in the embedding trie, the  address of its \tNode in memory can be used as the unique ID.

\item \underline{\textit{Retrieval}} Given a particular ID represented by a \tNode, we can easily follow its pointer $parentN$ step-by-step to retrieve the corresponding result.

\item \underline{\textit{Removal}}
To remove a result with a particular ID, we can remove its corresponding \tNode and decrease the $childCount$ of its parent node by 1. If $ChildCount$ of this parent node reaches 0, we remove this parent node. This process recursively affects the ancestors of the \tNode.

\end{itemize}




==> Outline/outline_1.tex <==
\section{RADS Architecture}
\label{sec:outline}

In this section, we first present an overview of the architecture of $\Pads$, followed by the $\Mur$ framework of $\Pads$, and finally a detailed  implementation of $\Mur$.

\subsection{Architecture Overview}

\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.5\textwidth]{Pictures/architecture}
\caption{RADS Architecture}
\label{fig:architecture}
\end{figure}

The architecture of $\Pads$ is shown in Figure~\ref{fig:architecture}.
%
{Given a query pattern $P$, within each machine, $\Pads$ first launches a process of single-machine enumeration (\sme) and a daemon thread, simultaneously. After \sme finishes, $\Pads$ launches a R-Meef thread subsequently. Note that the R-Meef threads of different machines may start at different time.}


\begin{itemize}[leftmargin=*]

\item \textbf{Single-Machine Enumeration}
%Single-machine subgraph enumeration algorithms have been well optimized, and most of them follow the backtracking approach and have small memory cost  \cite{DBLP:journals/pvldb/LeeHKL12}\cite{turboIso}\cite{boostIso}. 
The idea of \sme is to try to find a set of local embeddings using a single-machine algorithm, such as TurboIso\cite{turboIso}, which does not involve any distributed processing. The subsequent distributed process only has to find the remaining embeddings.  
%
This strategy can not only boost the overall enumeration efficiency but also significantly reduce the memory cost and communication cost of the subsequent distributed process.
{Moreover the local embeddings can be used to estimate the space cost of a {\em region group}, which will help to effectively control the memory usage (to be discussed in Section~\ref{sec:memoryControl}).}

We first define the concepts of {\em border distance} and {\em span}, which will be used to identify embeddings that can be found by \sme.
%First of all, we need to identify the embeddings that can be found by \sme.  For this we need the following two definitions.

\begin{defn}[Border Distance]
\label{defn:borderDia}
Given a graph partition $G_t$ and data vertex $v$ in $G_t$, the {\em border distance} of $v$ w.r.t $G_t$,  denoted as $\BD_{G_t}(v)$, is the minimum shortest distance between $v$ and any border vertex of $G_t$, that is
\begin{equation}
\BD_{G_t}(v) = \min \limits_{v' \in V_{G_t}^b} dist(v, v')
\end{equation}
where $dist(v, v')$ is the shortest distance between $v$ and $v'$.
\end{defn}


\begin{defn}[Span]
\label{defn:queryDia}
Given a query pattern $P$, the {\em span} of query vertex $u$, denoted as $\QD_{P}(u)$, is the maximum shortest distance between $u$ and any other vertex of $P$, that is
\begin{equation}
\QD_{P}(u) = \max \limits_{u' \in V_P} dist(u, u')
\end{equation}
\end{defn}

%Note that our definition of farness is slightly different from that of some other definitions, for exp
%is restricted to each query vertex, in contrast to the diameter of $P$ which is the maximum shortest distance between any pair of query vertices.


\begin{proposition}
\label{lem:diaEmbed}
Given a data vertex $v$ of $G_t$ and a query vertex  $u$ of $P$, if $ \QD_{P}(u)\leq \BD_{G_t}(v)$, then there will be no embedding $f$ of $P$ in $G$ such that $f(u)=v$, and $f(u')$ is not owned by $M_t$,  where $u' \in P$, $u' \neq u$.
\end{proposition}

Proposition~\ref{lem:diaEmbed} states that if the border distance of $v$  is not smaller than the span of query vertex $u$, there will be no cross-machine embeddings (i.e.,  embeddings where the query vertices are mapped to data vertices residing in different machines) which map $u$ to $v$. The proof of Proposition~\ref{lem:diaEmbed} is in the appendix.


Let $u_{start}$ be the starting query vertex (namely, the first query vertex to be mapped) and $C(u_{start})$ be the candidate vertex set of $u_{start}$ in $G_t$.
Let $C_1(u_{start})\subseteq C(u_{start})$ be the subset of candidates whose border distance is no less than the span of $u_{start}$. According to  Proposition~\ref{lem:diaEmbed}, any embedding that maps $u_{start}$ to a vertex in $C_1(u_{start})$ can be found using a single-machine subgraph enumeration algorithm over $G_t$, independent of other machines. In \Pads, the candidates in $C_1(u_{start})$ will be processed by \sme, and the other candidates will be processed by the subsequent distributed process. 
%
{The \sme process is simple, and we will next focus on the distributed process.  For presentation simplicity, from now on when we say a candidate vertex of $u_{start}$, we mean a candidate vertex in $C(u_{start})-C_1(u_{start})$, unless explicitly stated otherwise.}



%We discuss our method to compute and store the border distances of data vertices in Appendix~\ref{appendix:borderDia}.

\ignore{  Note in \sme, we will first compute a query execution plan whose pivot vertex of first decomposition unit will be used as the starting query vertex $u_{start}$.  The details of execution plan will be discussed in Section~\ref{sec:executionPlan}.}
%\vspace{2pt}

The distributed process consists of some daemon threads and the subgraph enumeration thread: 


\item \textbf{Daemon Threads} listen to requests from other machines and support four functionalities: \\
%
\textit{(1) verifyE} is to return the {\em edge verification} results for a given request consisting of vertex pairs. For example, given a request $\{(v_0, v_1)$, $(v_2, v_3)\}$  posted to $M_1$, $M_1$ will return $\{true, false\}$ if $(v_0, v_1)$ is an edge in $G_1$ while $(v_2, v_3)$ is not. \\
%
\textit{(2) fetchV} is to return the adjacency-lists of the requested vertices of the data graph. The requested vertices sent to machine $M_i$ must reside in $M_i$. \\
%
\textit{(3) checkR} is to return the number of unprocessed {\em region groups} (which is a group of candidate data vertices of the starting query vertex, see Section~\ref{subsec:rmeef}) of the local machine (i.e., the machine on which the thread is running). \\
%
\textit{(4) shareR} is to return an unprocessed region group of the local machine to the requester machine. \textit{shareR} will also mark the region group sent out as processed.

\item \textbf{R-Meef Thread}  is the core subgraph enumeration thread. \ignore{which employs a novel framework named $\Mur$ (\rmeef).} When necessary, the local $\Mur$ thread sends \textit{verifyE} requests and \textit{fetchV} requests to the Daemon threads located in other machines, and the other machines respond to these requests accordingly. 
    
Once a local machine finishes processing its own region groups, it will broadcast a \textit{checkR} request to the other machines.
Upon receiving the  numbers of unfinished region groups from other machines, it will send a \textit{shareR} request to the machine with the maximum number of unprocessed region groups. Once it receives a region group, it will process it on the local machine. \textit{checkR} and \textit{shareR} are for load balancing purposes only, and they will not be discussed further in this paper.
\end{itemize}

%We use $\Pads$ to refer to our distributed subgraph enumeration system as a whole, and use $\Mur$ to refer to the core framework and its implementation. %of the core of $\Pads$.

\subsection{The R-Meef Framework}
\label{subsec:rmeef}
%The architecture of our distributed subgraph enumeration system $\Pads$ has already been presented in the above subsection. The functions within the daemon thread are easy to understand, therefore we omit further details about them.

%Before presenting the  details of SubEnum, we first explain its underlying framework, which can be abstracted as $\Mur$(\textit{\textbf{r}egion-grouped \textbf{m}ulti-round \textbf{e}xpand and \textbf{a}ssemble based on verify $\&$ \textbf{f}ilter}), where the following definitions are important.

Before presenting the details of the $\Mur$ framework, we need the following definitions.

\begin{defn} [embedding candidate]
Given a partition $G_t$ of data graph $G$ located in machine $M_t$ and a query pattern $P$, an injective function $f_{G_t}$: $V_P$  $\rightarrow$  $V_{G}$ is called an {\em embedding candidate (EC)} of $P$  $w.r.t$ $G_t$ if for any edge $(u$, $u')$ $\in$ $E_{P}$, there exists an edge $( f_{G_t} (u)$, $f_{G_t}(u') )$ $\in$ $E_{G_t}$ provided either $f_{G_t} (u)$ $\in$ $V_{G_t}$ or $f_{G_t}(u')$ $\in$ $V_{G_t}$.
\end{defn}

We use \ecsb to denote the set of {\ec}s of $P$ $w.r.t$ $G_t$.
Note that for an \ec $f_{G_t}$ and a query vertex $u$,  $f_{G_t}(u)$ is not necessarily owned by $G_t$. That is, the adjacency-list of $f_{G_t}(u)$ may be stored in other machines. For any query edge $(u,u')$, an \ec only requires that the corresponding  data edge $( f_{G_t} (u)$, $f_{G_t}(u') )$ exists if at least one of $f_{G_t} (u)$ and $f_{G_t}(u')$  resides in $G_t$. Therefore, an \ec may not be an embedding.
%
Intuitively, the existence of the edge $(f_{G_t} (u), f_{G_t}(u'))$ can only be verified in $G_t$ if one of its end vertices resides in $G_t$. Otherwise the existence of the edge  cannot be verified in $M_t$, and we call such edges {\em undetermined} edges.

\begin{defn}
Given an \ec $f_{G_t}$ of query pattern $P$, for any edge $(u,u')\in E_P$, we say $(f_{G_t}(u), f_{G_t}(u'))$ is an \emph{undetermined edge} of $f_{G_t}$ if neither $f_{G_t}(u)$ nor $f_{G_t}(u')$ is in $G_t$.
\end{defn}


\begin{exmp}
Consider a partition $G_t$ of a data graph $G$ and a triangle query pattern $P$ where $V_P=\{u_0, u_1, u_2\}$. The mapping $f_{G_t}=$ $\{(u_0, v_0)$, $(u_0, v_1)$, $(u_0, v_2)\}$ is an \ec of $P$ in $G$ $w.r.t$ $G_t$ if $v_0 \in V_{G_t}$, $v_1 \in adj(v_0)$ and $v_2 \in adj(v_0)$ and neither $v_1$ nor $v_2$ resides in $G_t$. $(v_1, v_2)$ is an undetermined edge of $f_{G_t}$.
\end{exmp}

Obviously if we want to determine whether $f_{G_t}$ is actually an embedding of the query pattern, we have to verify its undetermined edges in other machines. For any undetermined edge $e$, if its two end vertices reside in two different machines, we can use either of them to verify whether $e \in E_G$ or not. To do that, we need to send a \textit{verifyE} request to one of the machines.

Note that it is possible that an undetermined edge is shared by multiple {\ec}s. To reduce network traffic, we do not send \textit{verifyE} requests once for each individual \ec, instead, we build an {\em edge verification index} (\evi) and use it to identify {\ec}s that share undetermined edges.  We assume each \ec is assigned an ID  (We will discuss how to assign such IDs and how to build \evi in Section~\ref{sec:embeddingTrie}).

%Next let us assume that we have an identification strategy such that each $f_{G_t}$ can be looked up by a unique ID. (We will discuss our identification strategy in Section~\ref{sec:invertedTrie}.)

\begin{defn}[edge verification index]
Given a set \ecsb of {\ec}s, the \emph{edge verification index (\evi)} of \ecsb is a key-value map  $\ei$ where
\begin{enumerate}
\item[(1)] for any tuple $(e, IDs)\in \ei$,
\begin{itemize}
\item the key $e$ is a vertex pair $(v, v')$.
\item the value $IDs$ is the set of IDs of the {\ec}s in \ecsb of which $e$ is an undetermined edge.
\end{itemize}
\item[(2)] for any undetermined edge $e$ of $f_{G_t} \in$ \ecsb, there exists a unique tuple in $\ei$ with $e$ as the key and the ID of $f_{G_t}$ in the value.
\end{enumerate}
\end{defn}

Intuitively, the \evi groups the {\ec}s that share each undetermined edge together.  It is straightforward to see:

\begin{proposition}
Given data graph $G$, query pattern $P$ and an edge verification index $\ei$, for any $(e, IDs) \in \ei$, if $e \notin E_{G}$, then none of the {\ec}s corresponding to $IDs$ can be an embedding of $P$ in $G$.
\end{proposition}

%We have explained  $f_{G_t}$, $\mathbb{R}_{G_t}(P)$ and \evi, which are key structures of the data flowing in the workflow of $\Mur$.
%We are now ready to define the execution plan which guides the workflow of $\Mur$.
%Before that, we present the definition of our query decomposition.


\ignore{
Recall that the striped graph $\overline{P}$ of $P$ is the graph obtained from $P$ by removing the original end vertices. In our approach, we process $\overline{P}$ first, and then attach the matches of the end vertices to the results of $\overline{P}$.
%
For any end vertex, its matches only depend on the matches of the query vertex attached to it and are independent with others. With the embeddings of $\overline{P}$ ready, to each of them, we can simply attach the possible combinations of the matches of end vertices one by one. Each result is a final embedding and can be output immediately. This will save us a lot of memory usage compared with directly processing $P$ where the intermediate results related to those end vertices have to be cached.
%
}

Like SEED and Twintwig, we decompose the pattern graph into small decomposition units.    

%We decompose the stripped query pattern $\sPattern$ into a set of decomposition units.

\begin{defn}[decomposition]
\label{defn:decomposition}
A decomposition of stripped query pattern $\sPattern=(V_{\sPattern}$, $E_{\sPattern})$ is a sequence of decomposition units $\decomp$ $=$ $(dp_0$, $\dots$, $dp_l)$ where every $dp_i \in $ $\decomp$ is a subgraph of $\sPattern$ such that

\begin{enumerate}

\item[(1)] The vertex set of $dp_i$ consists of a {\em pivot} vertex $\piv$ and a non-empty set $\lf$ of {\em leaf\footnote{In an abuse of the word ``leaf".} vertices}, all of which are vertices in $V_{\sPattern}$; and for every $u' \in \lf$, $(\piv, u') \in E_{\sPattern}$.


\item[(2)] The edge set of $dp_i$ consists of two parts,  $E_{dp_i}^{star}$  and $E_{dp_i}^{sib}$, where  $E_{dp_i}^{star}$ $=$ $\bigcup_{u' \in \lf}$ $\{(dp_i.\piv,$ $u')\}$
    is the set of edges between the pivot vertex and the leaf vertices, and
    $E_{dp_i}^{sib}$ $=$ $\bigcup_{u, u' \in dp_i.\lf}$ $\{(u, u')$ $\in$ $E_{\sPattern} \}$ is the set of edges between the leaf vertices.

\item[(3)] $\bigcup_{dp_i \in \decomp}(V_{dp_i}) = V_{\sPattern}$, and for $i<j$, $V_{dp_i}\cap dp_j.\lf=\emptyset$.
\end{enumerate}
\end{defn}

Note condition (3) in the above definition says the leaf vertices of each decomposition unit do not appear in the previous units.
Similar to the decompositions  in \cite{DBLP:journals/pvldb/LaiQLC15}and \cite{DBLP:journals/pvldb/LaiQLZC16}, our decomposition units cover all the vertices of $\sPattern$ and share no common edges with each other. However, our decomposition unit is not restricted to stars and cliques.  It is worth noting that $\bigcup_{dp_i \in \decomp}(E_{dp_i})$ may be a proper subset of $E_{\sPattern}$.


\begin{exmp}
\label{exmp:executionPlan}
Consider the query pattern in Figure~\ref{fig:runningExample1}(a). $u_7$ and $u_{10}$ are end vertices. By removing those end vertices, we can get the stripped pattern $\sPattern$ of $P$.  For $\sPattern$ we may have a decomposition $(dp_0$, $dp_1$, $dp_2$, $dp_3)$ where $dp_0.\piv$ $=$  $u_0$, $dp_0.\lf$ $=$ $\{u_1$, $u_2\}$, $dp_1.\piv$ $=$ $u_1$, $dp_1.\lf$ $=$ $\{u_3, u_4\}$, $dp_2.\piv$ $=$ $u_2$, $dp_2.\lf$ $=$ $\{u_5$, $u_6\}$, and  $dp_3.\piv$ $=$ $u_0$, $dp_3.\lf$ $=$ $\{u_8, u_9\}$. Note that the edge $(u_4$, $u_5)$ is not in any decomposition unit.
\end{exmp}


\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.45\textwidth]{Pictures/runningExmp1}
\caption{Running Example}
\label{fig:runningExample1}
\end{figure}


Given a decomposition $\decomp=(dp_0$,  $\dots$,  $dp_{l})$ of stripped pattern $\sPattern$, we define a sequence of \textit{sub-query} patterns $P_0, \ldots, P_l$, where $P_0$ = $dp_0$, and for $i>0$, $P_i$ consists of the union of $P_{i-1}$ and $dp_i$ together with the edges across the vertices of $P_{i-1}$ and $dp_i$, that is, $V_{P_i}$ = $\bigcup_{j \leq i} V_{dp_j}$, $E_{P_i}$ = $\bigcup_{j \leq i} $ $E_{P_j}$ $\cup$ $\{(u_i, u_j)\in E_P | u_i\in P_{i-1}, u_j\in dp_i.\lf\}$. Note that (a) none of the leaf vertices of $dp_i$ can be in $P_{i-1}$; and (b) $P_i$ is the subgraph of $P$ induced by the vertex set $V_{P_i}$, and $P_l =P$. We say $\decomp$ forms an {\em execution plan} if for every $i\in [1,l]$, the pivot vertex of $dp_i$ is in $P_{i-1}$\ignore{, and none of the leaf vertices of $dp_i$ is in $P_{i-1}$}. Formally, we have

\begin{defn}[execution plan]
\label{defn:executionPlan}
A decomposition $\decomp=(dp_0$,  $\dots$,  $dp_{l})$ of $\sPattern$ is  an {\em execution plan}($\joinplan$) if $dp_i.\piv$ $\in$ $V_{P_{i-1}}$ for all $i\in [1,l]$.
\end{defn}

For example, the decomposition in Example~\ref{exmp:executionPlan} is an execution plan.
%An execution plan provides a rough processing order for the query pattern $P$.

Let  $\joinplan=(dp_0$,  $\dots$,  $dp_{l})$ be an execution plan. For each $dp_i$, we define
\[ E_{dp_i}^{cro} = \{(u_i, u_j)\in E_P | u_i\in P_{i-1}, u_j\in dp_i.\lf\} (\mbox{for } i> 0)\]

We call the edges in  $E_{dp_i}^{star}$, $E_{dp_i}^{sib}$ and  $E_{dp_i}^{cro}$ the {\em expansion} edges, {\em sibling } edges, and {\em cross-unit} edges respectively. The sibling edges and cross-unit edges are both called {\em verification} edges.

Consider $dp_0$ in Example~\ref{exmp:executionPlan}, we have $E_{dp_0}^{sib}$=$\{(u_1, u_2)\}$, $E_{dp_0}^{cro}$=$\emptyset$. For $dp_2$, we have $E_{dp_2}^{sib}$=$\{(u_5, u_6)\}$, $E_{dp_2}^{cro}$=$\{(u_4, u_5)\}$.

\begin{proposition}
Given an execution plan $\joinplan=(dp_0$,  $\dots$,  $dp_{l})$ of stripped query pattern $\sPattern$, it holds that $|\bigcup_{dp_i \in \joinplan}(E_{dp_i}^{star})|$ = $(|V_{\sPattern}| - 1)$.
\end{proposition}


Intuitively, the  expansion edges of all the units form a spanning tree of pattern $\sPattern$. The verification  edges are the edges not in the spanning tree.





==> Outline/outline_assemble__algorithmmethod.tex <==


%\ignore{
%	The final results will be obtained when $P_l$ is evaluated in all machines (each machine computes a subset of the final embeddings, the union of which is the final set of embeddings).  %We will call the results of $P_0, \ldots, P_{l-1}$ the intermediate results.
%%
%	{\color{red}is it possible that the candidate set of $M_t$ is empty, or all candidates reside in one machine? Theoretically it is possible -- this is not considered in twinTwig either}
%}
%%
An execution plan provides a processing order for the query pattern $P$. In principle, a multi-round approach can be used to evaluate pattern $P$: each machine $M_t$ can evaluate $P_0$ in the first round, and based on the results obtained for $P_{i}$ in round $i$, it can evaluate the next pattern $P_{i+1}$ in the next round. The final results will be obtained when $P_l$ is evaluated in all machines (each machine computes a subset of the final embeddings, the union of which is the final set of embeddings).  In our approach, however, to reduce intermediate results and make the evaluation more efficient, we divide the evaluation of $P$ into two phases: expand and assemble. In the expand phase, we compute the embeddings of each individual decomposition unit; in the assemble phase, these embeddings will be assembled together to obtained the embeddings of $P$. More details will be given below.


%With the above concepts, we are ready to present the principles of $\Mur$ framework.
%
Given query pattern $P$, data graph $G$ and its partition $G_t$ within a machine $M_t$, $\Mur$ finds a set of embeddings of $P$ in $G_t$ based on the following:
%
\begin{enumerate}[leftmargin=*]


\item[(1)] \textit{\underline{Region-Grouped}}~  In our approach, each machine $M_t$ will evaluate $dp_0$ first, starting with the mapping of $dp_0.\piv$ to a candidate vertex that resides in $M_t$. If the number of candidate vertices is large, there is a possibility of generating too many intermediate results  (i.e., {\ec}s) if we process those candidate vertices together. To minimize the chance of memory crash, we divide the candidate vertex set of $dp_0.\piv$ into disjoint {\em region-groups}, and process each group sequentially and separately. The details will  be given in Section~\ref{??}.

%where $dp_0.\piv$ will be mapped to every candidate vertex of $dp_0.\piv$ that resides in $M_t$. Starting from each candidate vertex $v$, we may treat the part of the data graph as a \textit{region} where we can find all the embeddings with $dp_0.\piv$ mapped to $v$.
%
%When the number of such candidate vertices is large, there is a possibility of generating too many intermediate results (i.e., \ecs) if we process those candidate vertices together.
%
%\\
%In our approach, we divide the candidate vertex set of $dp_0.\piv$ into disjoint {\em region-groups} $\regiongroup=\{rg_0$, $\dots$, $rg_h\}$, and process each group sequentially and separately. The idea is to divide the workload into multiple independent processes so that the maximum intermediate results cached in memory can be limited. The purpose of this is to minimize the chance of memory crash.

\item[(2)] \textit{\underline{Multi-round expand and assemble}}  For each region-group, $\Mur$ launches two successive phases,\textit{expand} and \textit{assemble}, each of which is a multi-round process based on the execution plan $\joinplan$.
%
%
\begin{itemize}
\item \underline{\textit{Expand}}~ In the expand phase, $\Mur$ finds the embeddings of each decomposition unit in each machine $M_t$. The workflow of the expand phase in the $i^{th}$ round, in which we compute the embeddings of $dp_i$, is illustrated in Figure~\ref{fig:expand_phase}.


\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.4\textwidth]{pictures/expand_phase}
\caption{Workflow of expand phase in each round}
\label{fig:expand_phase}
\end{figure}

In Figure~\ref{fig:expand_phase}, $C_{G_t}(dp_i.\piv)$ represents the candidate vertices of the pivot vertex of $dp_i$. For the first round (i.e., round 0), $C(dp_0.\piv)$ is initialized as $\bigcup\{v | \deg(v) \geq deg(u)\}$ where $v$ is a  vertex residing in $M_t$.
%
 For round $i$ ($i>0$), assume $dp_i.v_{pivot} \in dp_j.\lf$ ($j<i$), then $C_{G_t}(dp_{i}.\piv)$ is the set of data vertices that are matched to $dp_i.\piv$ by the embeddings of $dp_j$. Formally,
\begin{equation}
C_{G_t}(dp_{i}.\piv)= \{f_{G_t}(dp_i.\piv) | f_{G_t} \in \mathbb{R}_{G_t}(dp_j) \}
\end{equation}
%Note that each vertex only appears once in $C_{G_t}(dp_{i}.\piv)$.


We expand from each candidate vertex $v$ $\in$ $C(dp_i.\piv)$ by searching its neighbourhood, and we find all the {\ec}s of $dp_i$ $w.r.t$ $G_t$ where $v$ is mapped to $dp_i.\piv$. It is worth noting that if $v$ does not reside in $M_t$, we have to fetch its adjacency-list from other machines. 
%\ignore{In order to reduce network traffic, we first gather those vertices that need to be fetched and then fetch their adjacency-lists together by sending a single $fetchV$ request.}

Once we have the set of {\ec}s \ecb{dp_i}, we store it compactly in a trie (referred to as {\em embedding trie} {\color{red} unit trie? expand trie?}) and build an EVI, then    
%we can easily build an $\evi$ from them. After that,
we launch a $verify~ \&$ $filter$ process to verify the undetermined edges of \ecb{dp_i} and filter out the failed {\ec}s. Note that the undetermined edges are the edges corresponding to $E_{dp_i}^{sib}$. This will generate the set \ecsp{dp_i} of all embeddings of $dp_i$ in each machine $M_t$.

The \ec trie and EVI will be discussed in Section~\ref{sec:embeddingTrie}. 

\vspace{2pt}
\item \underline{\textit{Assemble}} In the assemble phase, $\Mur$ finds the final embeddings of $P$ in each machine $M_t$ by assembling the embeddings of the decomposition units generated from the $expand$ phase. The workflow of assemble phase in the $i^{th}$ $(i \geq 1)$ round can be illustrated in Figure~\ref{fig:assemble_phase}.
\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.35\textwidth]{pictures/assemble_phase}
\caption{Workflow of assemble phase in each round}
\label{fig:assemble_phase}
\end{figure}

In Figure~\ref{fig:assemble_phase},  $\mathbb{R}_{G_t}(P_{i-1})$ represents the embeddings assembled and cached from the previous round. If it is the first round (i.e., round 0), $\mathbb{R}_{G_t}(P_{i-1})$ will be initialized as $\mathbb{R}_{G_t}(dp_0)$. For each $f_{G_t}$ $\in$ $\mathbb{R}_{G_t}(P_{i-1})$, we assemble $f_{G_t}$ with each embedding $f \in$ $\mathbb{R}_{G_t}(dp_i)$ where $f(dp_i.\piv)$ $=$ $f_{G_t}(dp_i.\piv)$ and there is no data vertex matched to different query vertices by $f$ and $f_{G_t}$. The assembling output is an \ec of $P_i$ $w.r.t$ $G_t$.

Once we have a set of {\ec}s \ecb{P_i}, we store them in a trie (referred to as {\em hyperembedding trie} {\color{red} cross-unit trie? assemble trie?}) and build an EVI,  then we  launch the $verify~\&$ $filter$ process to filter out failed {\ec}s. Here the undetermined edges are the edges corresponding to $E_{dp_i}^{cro}$. After this filtering step we will obtain all the embeddings of $P_i$ in each machine $M_t$. If it is the last round, that is, $i=l$, $\mathbb{R}_{G_t}(P_{i})$ is the set of final embeddings of $P$ in machine $G_t$.

\end{itemize}

\item[(3)] \textit{\underline{Verify $\&$ Filter}}
For each EVI, we send its keys, which are undetermined data edges, to other machines to verify their existence. One important assumption here is that each machine has a record of the ownership information (i.e., which machine a data vertex resides in) of all the vertices. This record can be constructed offline as a map whose size is $|V|$. After we get the verification results, each failed key indicates that the corresponding {\ec}s can be filtered out. 

\end{enumerate}







\subsection{Algorithm of SubEnum}
Next we look at the implementation of $\Mur$ as shown in Algorithm~\ref{algorithm:disSubEnum}.  Algorithm~\ref{algorithm:disSubEnum} is executed in each machine $M_t$ simultaneously and asynchronously.
%
\begin{algorithm}
\DontPrintSemicolon
\small
\SetAlgoLined
\KwIn{Query pattern $P$ and Data graph $G$ partitioned into $\{G_{1}, G_{2}, \dots, G_{m}\}$ located at $m$ machines from $M_{1}$ to $M_{m}$}
\KwOut{All embeddings of $Q$ in $G$}

\For{\textbf{each} machine $M_t$($1\leq t \leq m$) \textbf{simultaneously}}
{
	$\joinplan$ $\gets$ $executionPlan(P)$ \\
	
	$\regiongroup$=$\{rg_0 \dots rg_k\}$ $\gets$ $regionGroups\big(C(dp_0.\piv, M_t)\big)$ \\
		
	Init a list of embedding tries $\eTrie$, one for each $dp_i$  \\
	
	\For{\textbf{each} region-group $rg \in \regiongroup$}
	{	
		\For{round $i = 0$ to $|\joinplan| - 1$}
		{
			\If{$i = 0$}
			{
				$C_{G_t}(dp_0.\piv)$ $\gets$ $\{v|v \in G_t, deg(v) \geq deg(u)\}$ \\
			}
			\Else
			{
				Find $j$ such that $j<i$ and $dp_i.\piv \in V_{dp_j}$  \\
				\For{\textbf{each} $f \in $ $\eTrie$ $[j]$}
				{
					\If{$f(dp_i.\piv)$ $\notin$ $C_{G_t}(dp_i.\piv)$}
					{
						add $f(dp_i.\piv)$ to $C_{G_t}(dp_i.\piv)$ \\
					}
				}
                
				$fetchForeignV$($C_{G_t}(dp_i.\piv)$) \\		
			}
			
			[$\eTrie$, $\evi$] $\gets$ $expandETrie$($C_{G_t}(dp_i.\piv)$, $dp_i$) \\
			
			$\mathcal{R} \gets verifyForeignE(\evi)$      \\
			
			$\eTrie$[i] $\gets$ $filterFailedEmbed(\mathcal{R}, \eTrie)$  \\
		}
		
		Init hyper embedding trie $\hypTrie$ using $\eTrie$[0] \\
		\For{round $i = 1$ to $|\joinplan| - 1$}
		{
									
			[$\hypTrie$, $\evi$] $\gets$ $assembleHETrie($ $\eTrie[i]$, $\hypTrie$) \\
			$\mathcal{R} \gets verifyForeignE(\evi)$      \\
			$\hypTrie$ $\gets$ $filterFailedEmbed(\mathcal{R}, \hypTrie)$ \\
		}
		$outputFinalEmbed$($\hypTrie$) 
	}	
}

\caption{\sc SubEnum }
\label{algorithm:disSubEnum}
\end{algorithm}

\renewcommand\labelenumi{(\arabic{enumi})}
\renewcommand\theenumi\labelenumi
\begin{enumerate}[leftmargin=*]
\item Within each machine, we first compute an execution plan $\joinplan$ based on the given query pattern $P$ (Line 2). The execution plans computed in all machines are the same.
\item We group the candidate data vertices of $dp_0.\piv$ within $M_t$ into  region-groups (Line 3). For each region-group $rg$, a multi-round $expand$ phase (Line 4 to 17) and a multi-round $assemble$ phase (Line 18 to 22) are conducted.

%\begin{itemize}[leftmargin=*]
%\item  Within each machine, we first compute an execution plan $\joinplan$ based on the given query pattern $P$ (Line 2). The execution plans computed in all machines are the same.
%
%\item We group the candidate data vertices of $dp_0.\piv$ within $M_t$ into  region-groups (Line 3).
%For each region-group $rg$, a multi-round $expand$ phase (Line 4 to 17) and a multi-round $assemble$ phase (Line 18 to 24) are conducted.

%\item In Line 4, We use a list of cyclic embedding tries $\eTrie$s to save the generated embedding candidates for each decomposition unit, each one of which has a unique ID. In Line 18, We use a hyper embedding trie $\hypTrie$ to save the embedding candidates of $P_i$ assembled from the embeddings of decomposition units.
%%
%\ignore{We use intermediate results to refer those generated tries for short in the rest of the paper.}
%%
%We will give more details of cyclic and hyper embedding tries in Section~\ref{sec:embeddingTrie}.
%
%\item An edge verification index $\evi$ is used in each round of both the $expand$ and $assemble$ phases.

%\end{itemize}

%
\item \underline{\textit{Expand Phase}}~ In Line 8, we initialize the candidate vertices for $dp_0.\piv$ where each candidate must have a larger degree then $dp_0.\piv$. For each of the other rounds, $C_{G_t}(dp_i.\piv)$ is initialized as the set of data vertices matched to $dp_i.\piv$ in the previous rounds (Line 11 to 13). A function  $fetchForeignV$ is called to fetch foreign vertices from other machines (Line 14), and this function will find the data vertices in $C_{G_t}(dp_i.\piv)$ that need to be fetched, group them by the machines from which they can be fetched, and send fetchV requests to those machines. Upon receiving all fetched data vertices,  $expandETrie$ is called to get all the {\ec}s for $dp_i$ and save them in the corresponding trie $\eTrie[i]$. An edge verification index $\evi$ is built along the way (Line 15). After that, if there are undetermined edges, a function  $verifyForeignE$ will be called to send edge verification requests to other machines (Line 16). Upon receiving the verification results $\mathcal{R}$, failed \ec will be filtered out from $\eTrie$, and what left are the embeddings of $dp_i$.

\item \underline{\textit{Assemble Phase}}~
In Line 18, we initialize a hyper embedding trie $\hypTrie$, which is initially a single-level trie where each node represents an embedding from $\eTrie$[0]. From round 1 to the last round, the $\hypTrie$ will be grown by assembling its embeddings with the embeddings of $dp_i$ stored in $\eTrie$[i]. This process is done by concatenating each $f\in \hypTrie$ and each embedding $f'\in \eTrie[i]$ that satisfy $f(dp_i.\piv)$=$f'(dp_i.\piv)$ and $f$ and $f'$ do not map different query vertices to the same data vertex. An edge verification index $\evi$ will be built along the way, using which edge verification requests will be sent to other machines (if necessary) by calling $verifyForeignE$. Upon receiving the verification result, the failed embedding candidates in $\hypTrie$ will be removed (Line 22).

%\item[(4)] \underline{\textit{Final Output}}
When the $assemble$ phase is completed, we will output the embeddings of $P$ in $M_t$ found in this region-group. Note that the final embeddings are compressed in the tries $\eTrie$ and $\hypTrie$, and a function  $outputFinalEmbed$ needs to be called to output those final embeddings (Line 23).
\end{enumerate}
%
%We will present more details for the sub-functions refereed in Algorithm~\ref{algorithm:disSubEnum} in following sections. To have an intuitive understanding, let us study the following example:
\begin{exmp}
Consider the query pattern $P$ and the data graph $G$ in Figure~\ref{fig:runningExample1}, the vertices marked with red dash border are owned by $M_0$ and the other vertices reside in $M_1$. We use the execution plan given in Example~\ref{exmp:executionPlan}. We assume the preserved orders due to symmetry breaking are: $u_1<u_2$.


\emph{\textbf{Line 1 to 4:}} There are one vertex $\{v_0\}$ in $M_0$ and two vertices $\{v_9, v_{10}\}$ in $M_1$ with a degree not smaller than that of $dp_0.\piv$. Therefore in $M_1$, we have $C_{G_1}(dp_0.\piv)$ $=$ $\{v_0\}$ and in $M_2$ we have $C_{G_2}(dp_0$.$\piv)$ $=$ $\{v_9$, $v_{10}\}$.  After grouping, assume we have $\regiongroup=\{rg_0\}$ where $rg_0=\{v_0\}$ in $M_1$  and $\regiongroup=\{rg_0, rg_1\}$ where $rg_0=\{v_9\}$ and $rg_1=\{v_{10}\}$ in $M_2$.

\emph{\textbf{Line 6 to 17:}} Consider the region-group $rg_0$ in $M_1$, we first match $v_0$ to $dp_0.\piv$. Expanding from $v_0$, we may have embedding candidates including but not limited to $f_{G_1}$ $=$ $\{(u_0, v_0)$, $(u_1, v_1)$, $(u_2, v_2)$, $(u_7, v_7)\}$, $f_{G_1}'$ $=$ $\{(u_0, v_0)$, $(u_1, v_1)$, $(u_2, v_8)$, $(u_7, v_7)\}$ and $f_{G_1}''$ $=$ $\{(u_0, v_0)$, $(u_1, v_8)$, $(u_2, v_9)$, $(u_7, v_7)\}$. All these three candidate embeddings are compressed in a $\eTrie$.
%
The edges $(v_1$, $v_8)$ and $(v_8$, $v_9)$ cannot be determined in $M_1$. Therefore, we put $\{(v_1, v_8), <f_{G_1}'>\}$ and $\{(v_8, v_9), <f_{G_1}''>\}$ into $\evi$. There is no undetermined edges in $f_{G_1}$. After verification of $\evi$, a false returned for $(v_1$, $v_8)$, therefore $f_{G_1}'$ will be removed from $\eTrie$, the left will be assigned to $\eTrie$s[0].
%
In the next round with unit $dp_1$, we have $C_{G_t}(dp_1.\piv)$=$\{v_1$, $v_8$ $\}$. Since none of $C_{G_t}(dp_1.\piv)$ resides in $M_1$, we will fetch the adjacency-lists for those vertices to $M_1$. After that we expand each of $C_{G_t}(dp_1.\piv)$, we can get all the embedding candidates of $dp_1$ within $M_1$. Following the above process, after processing the last round of expand phase, the embeddings of every unit in machine $M_1$, starting from candidates of this region-group,  will be saved in $\eTrie$s.

\emph{\textbf{Line 18 to 24:}}  Upon having the embeddings of each unit in $M_t$, let us just consider $f_1 \in $ $\eTrie$s$[0]$, $f_2 \in $ $\eTrie$s$[1]$, $f_3 \in $ $\eTrie$s$[2]$ and $f_3 \in $ $\eTrie$s$[3]$., where $f_1$ $=$ $\{(u_0, v_0)$, $(u_1, v_1)$, $(u_2, v_2)$, $(u_7, v_7)\}$, $f_1$ $=$ $\{(u_1, v_1)$, $(u_3, v_3)$, $(u_4, v_4)\}$, $f_2$ $=$ $\{(u_2, v_2)$, $(u_5, v_5)$, $(u_6, v_6)\}$ and $f_3$ $=$ $\{(u_0, v_0)$, $(u_8, v_8)$, $(u_9, v_9)\}$. To get the embedding candidates of $P_1$ in first round, we assemble $f_1$ with $f_2$ where the data edge $(v_3$, $v_7)$ mapping to the verification edge $(u_3$, $u_7)$ can be verified as true locally and there is no other data vertices used twice. Then the assembled embedding $f_1$ $\leftarrow$ $f_2$ will be compressed in $\hypTrie$. Later on, it will be assembled with $f_3$ and $f_4$. Finally we have $f_1$ $\leftarrow$ $f_2$ $\leftarrow$ $f_3$ $\leftarrow$ $f_4$ in $\hypTrie$. To output this final embedding of $P$ in $M_t$, we need to stretch each embedding ID within $\hypTrie$ by referring its actual embedding content within $\eTrie$s.

\end{exmp}



==> Outline/outline_assemble_method_framework.tex <==


%\ignore{
%	The final results will be obtained when $P_l$ is evaluated in all machines (each machine computes a subset of the final embeddings, the union of which is the final set of embeddings).  %We will call the results of $P_0, \ldots, P_{l-1}$ the intermediate results.
%%
%	{\color{red}is it possible that the candidate set of $M_t$ is empty, or all candidates reside in one machine? Theoretically it is possible -- this is not considered in twinTwig either}
%}
%%
An execution plan provides a processing order for the query pattern $P$. In principle, a multi-round approach can be used to evaluate pattern $P$: each machine $M_t$ can evaluate $P_0$ in the first round, and based on the results obtained for $P_{i}$ in round $i$, it can evaluate the next pattern $P_{i+1}$ in the next round. The final results will be obtained when $P_l$ is evaluated in all machines (each machine computes a subset of the final embeddings, the union of which is the final set of embeddings).  In our approach, however, to reduce intermediate results and make the evaluation more efficient, we divide the evaluation of $P$ into two phases: expand and assemble. In the expand phase, we compute the embeddings of each individual decomposition unit; in the assemble phase, these embeddings will be assembled together to obtained the embeddings of $P$. More details will be given below.


%With the above concepts, we are ready to present the principles of $\Mur$ framework.
%
Given query pattern $P$, data graph $G$ and its partition $G_t$ within a machine $M_t$, $\Mur$ finds a set of embeddings of $P$ in $G_t$ based on the following:
%
\begin{enumerate}[leftmargin=*]


\item[(1)] \textit{\underline{Region-Grouped}}~  In our approach, each machine $M_t$ will evaluate $dp_0$ first, starting with the mapping of $dp_0.\piv$ to a candidate vertex that resides in $M_t$. If the number of candidate vertices is large, there is a possibility of generating too many intermediate results  (i.e., {\ec}s) if we process those candidate vertices together. To minimize the chance of memory crash, we divide the candidate vertex set of $dp_0.\piv$ into disjoint {\em region-groups}, and process each group sequentially and separately. The details will  be given in Section~\ref{??}.

%where $dp_0.\piv$ will be mapped to every candidate vertex of $dp_0.\piv$ that resides in $M_t$. Starting from each candidate vertex $v$, we may treat the part of the data graph as a \textit{region} where we can find all the embeddings with $dp_0.\piv$ mapped to $v$.
%
%When the number of such candidate vertices is large, there is a possibility of generating too many intermediate results (i.e., \ecs) if we process those candidate vertices together.
%
%\\
%In our approach, we divide the candidate vertex set of $dp_0.\piv$ into disjoint {\em region-groups} $\regiongroup=\{rg_0$, $\dots$, $rg_h\}$, and process each group sequentially and separately. The idea is to divide the workload into multiple independent processes so that the maximum intermediate results cached in memory can be limited. The purpose of this is to minimize the chance of memory crash.

\item[(2)] \textit{\underline{Multi-round expand and assemble}}  For each region-group, $\Mur$ launches two successive phases,\textit{expand} and \textit{assemble}, each of which is a multi-round process based on the execution plan $\joinplan$.
%
%
\begin{itemize}
\item \underline{\textit{Expand}}~ In the expand phase, $\Mur$ finds the embeddings of each decomposition unit in each machine $M_t$. The workflow of the expand phase in the $i^{th}$ round, in which we compute the embeddings of $dp_i$, is illustrated in Figure~\ref{fig:expand_phase}.


\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.4\textwidth]{pictures/expand_phase}
\caption{Workflow of expand phase in each round}
\label{fig:expand_phase}
\end{figure}

In Figure~\ref{fig:expand_phase}, $C_{G_t}(dp_i.\piv)$ represents the candidate vertices of the pivot vertex of $dp_i$. For the first round (i.e., round 0), $C(dp_0.\piv)$ is initialized as $\bigcup\{v | \deg(v) \geq deg(u)\}$ where $v$ is a  vertex residing in $M_t$.
%
 For round $i$ ($i>0$), assume $dp_i.v_{pivot} \in dp_j.\lf$ ($j<i$), then $C_{G_t}(dp_{i}.\piv)$ is the set of data vertices that are matched to $dp_i.\piv$ by the embeddings of $dp_j$. Formally,
\begin{equation}
C_{G_t}(dp_{i}.\piv)= \{f_{G_t}(dp_i.\piv) | f_{G_t} \in \mathbb{R}_{G_t}(dp_j) \}
\end{equation}
%Note that each vertex only appears once in $C_{G_t}(dp_{i}.\piv)$.


We expand from each candidate vertex $v$ $\in$ $C(dp_i.\piv)$ by searching its neighbourhood, and we find all the {\ec}s of $dp_i$ $w.r.t$ $G_t$ where $v$ is mapped to $dp_i.\piv$. It is worth noting that if $v$ does not reside in $M_t$, we have to fetch its adjacency-list from other machines. 
%\ignore{In order to reduce network traffic, we first gather those vertices that need to be fetched and then fetch their adjacency-lists together by sending a single $fetchV$ request.}

Once we have the set of {\ec}s \ecb{dp_i}, we store it compactly in a trie (referred to as {\em embedding trie} {\color{red} unit trie? expand trie?}) and build an EVI, then    
%we can easily build an $\evi$ from them. After that,
we launch a $verify~ \&$ $filter$ process to verify the undetermined edges of \ecb{dp_i} and filter out the failed {\ec}s. Note that the undetermined edges are the edges corresponding to $E_{dp_i}^{sib}$. This will generate the set \ecsp{dp_i} of all embeddings of $dp_i$ in each machine $M_t$.

The \ec trie and EVI will be discussed in Section~\ref{sec:embeddingTrie}. 

\vspace{2pt}
\item \underline{\textit{Assemble}} In the assemble phase, $\Mur$ finds the final embeddings of $P$ in each machine $M_t$ by assembling the embeddings of the decomposition units generated from the $expand$ phase. The workflow of assemble phase in the $i^{th}$ $(i \geq 1)$ round can be illustrated in Figure~\ref{fig:assemble_phase}.
\begin{figure}[htbp!]
\small
\centering
\includegraphics[width=0.35\textwidth]{pictures/assemble_phase}
\caption{Workflow of assemble phase in each round}
\label{fig:assemble_phase}
\end{figure}

In Figure~\ref{fig:assemble_phase},  $\mathbb{R}_{G_t}(P_{i-1})$ represents the embeddings assembled and cached from the previous round. If it is the first round (i.e., round 0), $\mathbb{R}_{G_t}(P_{i-1})$ will be initialized as $\mathbb{R}_{G_t}(dp_0)$. For each $f_{G_t}$ $\in$ $\mathbb{R}_{G_t}(P_{i-1})$, we assemble $f_{G_t}$ with each embedding $f \in$ $\mathbb{R}_{G_t}(dp_i)$ where $f(dp_i.\piv)$ $=$ $f_{G_t}(dp_i.\piv)$ and there is no data vertex matched to different query vertices by $f$ and $f_{G_t}$. The assembling output is an \ec of $P_i$ $w.r.t$ $G_t$.

Once we have a set of {\ec}s \ecb{P_i}, we store them in a trie (referred to as {\em hyperembedding trie} {\color{red} cross-unit trie? assemble trie?}) and build an EVI,  then we  launch the $verify~\&$ $filter$ process to filter out failed {\ec}s. Here the undetermined edges are the edges corresponding to $E_{dp_i}^{cro}$. After this filtering step we will obtain all the embeddings of $P_i$ in each machine $M_t$. If it is the last round, that is, $i=l$, $\mathbb{R}_{G_t}(P_{i})$ is the set of final embeddings of $P$ in machine $G_t$.

\end{itemize}

\item[(3)] \textit{\underline{Verify $\&$ Filter}}
For each EVI, we send its keys, which are undetermined data edges, to other machines to verify their existence. One important assumption here is that each machine has a record of the ownership information (i.e., which machine a data vertex resides in) of all the vertices. This record can be constructed offline as a map whose size is $|V|$. After we get the verification results, each failed key indicates that the corresponding {\ec}s can be filtered out. 

\end{enumerate}


==> Paper-Info/paper-info-sigmod.tex <==

\title{Fast and Robust Distributed Subgraph Enumeration}


\author{Xuguang Ren}
\affiliation{%
  \institution{Griffith University}
  \country{Australia}
}
\email{x.ren@griffith.edu.au}


\author{Junhu Wang}
\affiliation{%
  \institution{Griffith University}
  \country{Australia}
}
\email{j.wang@griffith.edu.au}


\author{Wook-Shin Han}
\affiliation{%
  \institution{POSTECH}
  \country{Public of Korea}
}
\email{wshan@dblab.postech.ac.kr}


\author{Jeffrey Xu Yu}
\affiliation{%
  \institution{The Chinese University of Hong Kong}
  \country{China}
}
\email{yu@se.cuhk.edu.hk}


==> Reference/reference-sigmod.tex <==
% ********************************** Bibliography ******************************
\bibliographystyle{ACM-Reference-Format}
\bibliography{Reference/reference}  % reference.bib is the name of the Bibliography in this case 

==> RelatedWork/relatedWork_backup.tex <==
\section{Related Work}
\label{sec:previousWork}


\ifpdf
    \graphicspath{{Chapter4/}}
\else
    \graphicspath{{Chapter4/}}
\fi


In this section, we extend the discussion of existing distributed subgraph enumeration solutions in Section~\ref{sec:introduction} and highlight the differences between them and our work. We classify them into three categories by their main techniques: \textit{Multi-round Join-oriented},  \textit{Exchanging Data Vertices}, and \textit{Compression}.

\subsection{Multi-round Join-oriented}

The state-of-the-art distributed subgraph enumeration solutions \cite{plantenga2013inexact}\cite{lai2015scalable}\cite{lai2017scalable} follow a multi-round join-oriented approach. They first decompose the query pattern into small \emph{join units} (a subgraph of the query pattern) and then launches multiple rounds of joins to get all the embeddings, whose process can be formulated as:
\begin{equation}
\mathbb{R}(P) = \mathbb{R}(p_0)  \Join  \mathbb{R}(p_1) \Join  \dots  \Join  \mathbb{R}(p_n).
\end{equation}
where $\mathbb{R}(p_i)$ denotes the embeddings of $p_i$ in data graph $G$.
%

\ignore{
Applying a two-way join, it is easy to see that there are exactly $n$ rounds in the whole procedure and  the $i^{th}$ round can be formulated as:
\begin{equation}
R(P_i)=R(P_{i}^l) \Join R(P_{i}^r)
\end{equation}
where $P_{i}^l$ and $P_{i}^r$ are called the left and right \emph{join elements} respectively. Either left or right element can be a  join unit or a \emph{join union} which is the union from several join units. }

The most critical problem of the above join-oriented approach is that a huge number of intermediate results will be generated and they may quickly drain the memory. Secondly, those intermediates need to be exchanged in each round, leading to heavy network communication and therefore, a huge network latency.


One more issue is that this approach inherits the intermediate latency of using join to solve subgraph enumeration.
Compared with join-oriented approach, the backtracking based method does not generate any intermediate results therefore has no such latency. Although the backtracking based TurboIso \cite{turboIso} has proved much faster than a typical join-oriented approach \cite{stw}, it is hard to determine whether the intermediate latency is a big problem because of other filtering and pruning techniques used in \cite{turboIso}. We better demonstrated this issue by comparing the performance of join-oriented approach with backtracking approach through a triangles listing task which avoids the effects of any auxiliary techniques. In our experiment, we show that the backtracking method outperformed join-oriented approach by 10 times in real datasets as shown in experiment~\ref{sec:experimentTriangleListing}.

Aiming to relieve the intermediate letancy of \cite{lai2015scalable}\cite{lai2017scalable}, the SubEnum thread of $\Pads$ utilizes an $\Mur$ approach which verifies and filters out the failed embedding candidates as early as possible. The intermediate latency is significantly reduced.

Similar to \cite{lai2015scalable}\cite{lai2017scalable}, $\Pads$ still generates some intermediate embeddings. However, we propose an inverted trie structure to effectively compress those intermediates. More importantly, we introduce a grouping strategy which divides the data candidates into region groups so that we can  process each group sequentially and separately. The maximum number of intermediate results of each  group is much smaller than the sum of processing all groups together. The ability to tune the peak number of intermediate results significantly increases the flexibility of our approach.

In contrast to \cite{lai2015scalable}\cite{lai2017scalable}, we do not send any intermediate results which can be quite explosive. Instead, we exchange edges that are need to be verified and adjacent-lists that are required (more details in next subsection), both of which are bounded by $|E|$.



\ignore{
Consider a distributed environment with $m$ machines and each machine holds a partition(\textit{a.k.a.} a part) of the data graph, the $i^{th}$ round in generalized two-way join procedure  is presented in the  following three phases.

\begin{itemize}
\item[(1)] \textit{Candidate Enumeration}: Given the join elements $P_{i}^l$, $P_{i}^r$, each machine $M_t$ will compute the embeddings for $P_{i}^l$ in $M_t$, say $R_{M_t}(P_{i}^l) = <f_1^l, f_2^l \dots >$; and  for $P_{i}^r$ in $M_t$,  say $R_{M_t}(P_{i}^r) = <f_1^r, f_1^r,  \dots>$, respectively.
\item[(2)] \textit{Group $\&$ Distribute}:  Upon all the machine finished candidate enumeration,  Both the sets of embeddings of $P_{i}^l$ and $P_{i}^r$ will be grouped by group keys $\mathcal{JK} = \{u_1, u_2, \dots\}$,  which are the data vertices that matched to the common query vertices of them, \textit{i.e.} $\mathcal{JK}=$ $V(P_{i}^l) \cap V(P_{i}^r)$. After that, the two embedding groups, one from $P_{i}^l$ and one from $P_{i}^r$, will be further grouped together, leading to a sets of key-value pairs of join candidates, one of which looks like: \begin{center}
$[key=<f_1^l(u_1), f_1^l(u_2),  \dots >, value=\{<f_1^l, f_2^l, \dots, >, <f_1^r,  f_2^r, \dots \}]$.
\end{center}
Then the key-value pairs will be distributed into the machines where any single key-value pair is assigned to the only one machine.

\item[(3)] \textit{Natural Join}: Each machine will launch a natural join process to each key-value pair candidates assigned to it. Any combination of $f_x^l$ and $f_y^l$ will generate a join result if they do not share any other matched data vertices.
\end{itemize}
}






\subsection{Exchanging Data Vertices}
The distributed subgraph enumeration solutions that choose to exchange data vertices instead of intermediate results include \cite{afrati2013enumerating}\cite{fan2017big}. By saying exchanging data vertices, we mean exchanging the adjacency-list of those vertices.  Both \cite{afrati2013enumerating} and \cite{fan2017big} follow a single-round style where, for any specific machine, it has to fetch a large set of data vertices from other machines. A fatal issue of these solutions is that the graph data held within each machine easily drains the memory of a single machine.

Similar to \cite{afrati2013enumerating}\cite{fan2017big}, $\Pads$ chooses to exchange data vertices. Differently, $\Pads$ uses a multi-round approach so that the data vertices exchanged are divided into multiple-rounds.  Instead of coping data vertices blindly, we also introduce maximum-caching strategy which releases previously fetched/used data  vertices when  it nearly drains the memory or has reached a given threshold. Those strategies grant us the ability to control the peak number of data vertices held in memory during the process.

Moreover, for non-spanning tree query edges, to determine whether some particular data edges (which cannot be verified locally) can be matched to them, we do not fetch related data vertices to the local machine. Instead, we send those edges to be verified to other machines and get the verification results from them. Sending particular edges and verification results is more lightweight than sending data vertices. This technique significantly reduces the workload that needs network communication.

\subsection{Compression}
Aiming to solve the output-crisis of the subgraph enumeration, \cite{qiao_sub} introduced a compression strategy to compress the output embeddings. By pre-indexing all the cliques of the data graph, \cite{qiao_sub} also proposed a distributed enumeration solution. Although \cite{qiao_sub} achieved some success in speeding up the subgraph enumeration process, it has to admit that its index is quite large (as shown in Table~\ref{t:qiao_index}.), which not only takes a large storage space but also increases the overhead of maintaining, especially when the data graph is frequently updated. This issue dramatically drops the practicality of \cite{qiao_sub}. In contrast, our approach does not need any auxiliary index except for the original data graph.

\begin{table}[h]
    \caption{Illustration of the Index Size}
	\centering
	\small
	\label{t:qiao_index}
 	\begin{tabular}{|c|c|c|c|c|}
    \hline
     \textbf{Dataset($G$)} & Original File Size & Index File Size \\ \hline \hline
   	 \textbf{DBLP}   & 13M   & 210M   \\ \hline
     \textbf{RoadNet} & 87M   & 569M     \\ \hline   	
   	 \textbf{LiveJournal}   & 501M   & 6.5G   \\ \hline
   	 \textbf{UK}   & 501M   & 6.5G   \\ \hline
	\end{tabular}
\end{table}

Compare with 
\cite{DBLP:journals/tjs/FeherAVML17}
\cite{DBLP:conf/sigmod/FanLLXYYX18}







==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
